A Non-commutative Extension of Lee-Seung's Algorithm for Positive Semidefinite Factorizations

Given a matrix $X\in \mathbb{R}_+^{m\times n}$ with nonnegative entries, a Positive Semidefinite (PSD) factorization of $X$ is a collection of $r \times r$-dimensional PSD matrices $\{A_i\}$ and $\{B_j\}$ satisfying $X_{ij}= \mathrm{tr}(A_i B_j)$ for all $\ i\in [m],\ j\in [n]$. PSD factorizations are fundamentally linked to understanding the expressiveness of semidefinite programs as well as the power and limitations of quantum resources in information theory. The PSD factorization task generalizes the Non-negative Matrix Factorization (NMF) problem where we seek a collection of $r$-dimensional nonnegative vectors $\{a_i\}$ and $\{b_j\}$ satisfying $X_{ij}= a_i^\top b_j$, for all $i\in [m],\ j\in [n]$ -- one can recover the latter problem by choosing matrices in the PSD factorization to be diagonal. The most widely used algorithm for computing NMFs of a matrix is the Multiplicative Update algorithm developed by Lee and Seung, in which nonnegativity of the updates is preserved by scaling with positive diagonal matrices. In this paper, we describe a non-commutative extension of Lee-Seung's algorithm, which we call the Matrix Multiplicative Update (MMU) algorithm, for computing PSD factorizations. The MMU algorithm ensures that updates remain PSD by congruence scaling with the matrix geometric mean of appropriate PSD matrices, and it retains the simplicity of implementation that Lee-Seung's algorithm enjoys. Building on the Majorization-Minimization framework, we show that under our update scheme the squared loss objective is non-increasing and fixed points correspond to critical points. The analysis relies on Lieb's Concavity Theorem. Beyond PSD factorizations, we use the MMU algorithm as a primitive to calculate block-diagonal PSD factorizations and tensor PSD factorizations. We demonstrate the utility of our method with experiments on real and synthetic data.

==> manuscript PSD case: arxiv/macros.tex <==
\usepackage{physics}
\usepackage{mathtools}
\usepackage{color}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage[nothing]{algorithm}
\usepackage{algorithmic}
     
\usepackage{amsmath}
%\renewcommand{\thealgorithm}{}
\usepackage[pdftex]{graphicx}
\usepackage{hyperref}


\newcommand{\sfT}{\top}
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\bbS}{\mathbb{S}}
\def\bal{\begin{aligned}}
\def\eal{\end{aligned}}
\newcommand{\psdrank}{\mathrm{psd}\textnormal{-rank}}

\newcommand{\mca}{\mathcal{A}}
\newcommand{\mcb}{\mathcal{B}}

\newcommand{\mcx}{\mathcal{X}}
\newcommand{\mcs}{\mathcal{S}}




\newcommand{\bo}{B_{\mathrm{old}}}
\newcommand{\bn}{B_{\mathrm{new}}}
\newcommand{\ao}{A_{\mathrm{old}}}
\newcommand{\an}{A_{\mathrm{new}}}

\newcommand{\sbo}{b^{\mathrm{old}}}
\newcommand{\sbn}{b^{\mathrm{new}}}
\newcommand{\sao}{a^{\mathrm{old}}}
\newcommand{\san}{a^{\mathrm{new}}}


\usepackage{color}

% Theorem environments
\newtheorem{theorem}{Theorem}[]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}

\theoremstyle{definition}
\newtheorem*{definition}{Definition}

\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\newtheorem*{example}{Example}

\newcommand{\aff}{\mathrm{aff}}
\newcommand{\ca}{\mathcal{A}}
\newcommand{\lqqd}{L(\R^{q \times q},\R^d)}
\newcommand{\R}{\mathbb{R}}

\newcommand{\bb}{\mathbf{b}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}

\newcommand{\psd}{\mathbb{S}_+}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\p}{\partial}
\newcommand{\sub}{\subseteq}
\newcommand{\lam}{\lambda}
\newcommand{\calf}{\mathcal{F}}
\newcommand{\face}{\triangleleft}
\newcommand{\amin}{\mathrm{argmin}}
\DeclareMathOperator{\dee}{d}
\DeclareMathOperator{\vect}{vec}
\DeclareMathOperator{\sgn}{sgn}
\DeclarePairedDelimiterX{\inn}[2]{\langle}{\rangle}{#1, #2}

\DeclareMathOperator{\new}{{\rm new}}
\DeclareMathOperator{\old}{{\rm old}}
\DeclareMathOperator{\dom}{{\rm dom}}
\newcommand{\vecc}{\mathrm{vec}} 

\DeclareMathOperator{\bnew}{B_{\mathrm{new}}}
\DeclareMathOperator{\bol}{B_{\mathrm{old}}}
\DeclareMathOperator{\cala}{\mathcal{A}}

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}


==> manuscript PSD case: arxiv/sec_checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage

\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerNo{}  
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}  %Our work is foundational and it informs the development for other machine learning frameworks such as neural networks (and especially CNNs).  We have decided to not include a discussion on potential societal impacts because (i) the discussion will be highly speculative, which distracts from the important purpose such discussions serve, and (ii) future downstream applications that build on our framework is the most reasonable 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}  The proof of Theorem \ref{LSstylethm} is in the main body.  It relies on Lemma \ref{thm:domination_general}, which is stated and proved in the Appendix.  The proof of Theorem \ref{fixedpointsthm} is found in the Appendix.
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}  The essential instructions are provided in the numerical experimental section.  The code will be uploaded to an online repository at a later date. 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}  An important feature of the MMU (our) algorithm we propose is that it does \emph{not} require a tuning parameter.  In the numerical experiment on the CBCL Face dataset, the choice of parameters were such that the number of degrees of freedom in all three methods are similary (either 27 or 28).
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}  The PSD factorization task is non-convex so the performance of any algorithm is dependent on initialization.  We describe the error bars (indirectly) in our plot in Figure \ref{fig:distancematrx_errors}.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}  The experiments were conducted on a laptop, and we briefly state the specifications in the mainbody.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} We used the CBCL Face Dataset \cite{CBCL}.
  \item Did you mention the license of the assets?
    \answerNo{}  We do not mention the license because it appears to be customized.  Nevertheless the license permits use of the dataset for academic research, and can be found on the cited URL.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}



==> manuscript PSD case: arxiv/sec_domination.tex <==

\section{Proof of the domination property}\label{algorithmic}
In this section we prove  the  domination property, which is the last remaining ingredient in the proof of Theorem \ref{LSstylethm}.
% showing that the identified functions are valid auxilliary functions, thus establishing the validity of our approach. 



\begin{lemma} \label{thm:domination_general}
Fix $r\times r$ positive definite matrices $A_1,\ldots,A_m$ and consider the linear mapping 
	 	\begin{equation*}
	\mathcal{A} : \mathbb{S}^{r} \rightarrow \mathbb{R}^{m} \text{ where } Z\mapsto \left(
	\langle A_1,Z \rangle, \ \ldots \ 
	,\langle A_m,Z \rangle
	 \right).
\end{equation*}
 Moreover, fix an $r\times r$ positive definite matrix   $B$  and set
			$$W = [\mathcal{A}^{\sfT} \mathcal{A}] (B)\#B^{-1}.$$ 
Then, we have that
	\begin{equation}\label{eq:main}
		\langle Z, WZW \rangle \geq \langle Z, [\mathcal{A}^{\sfT} \mathcal{A}] (Z) \rangle,  \text{ for all } Z \in \mathbb{S}^{r}.
	\end{equation}
\end{lemma}
\begin{proof}
First note that $W$ is well-defined as  $[\mathcal{A}^{\sfT} \mathcal{A}] (B)=\sum_{k=1}^m\la A_k,B\ra A_k$ is positive definite. First,  we  reduce the theorem to the special case  where $B=I$.
For this, define the linear map 
$$\tilde{\mathcal{A}} : \mathbb{S}^{r} \rightarrow \mathbb{R}^{m}, \quad  Z \mapsto  \mathcal{A}(B^{1/2}ZB^{1/2}).$$
  Noting that 
$$\tilde{\mathcal{A}}(I)= \cala(B) \ \text{ and } \ \tilde{\mathcal{A}}^\sfT(Z)=B^{1/2}\cala^\sfT(Z)B^{1/2},$$
it follows that 
	\begin{equation*}
		\begin{aligned}
			W & = [\mathcal{A}^{\sfT} \mathcal{A}] (B)\#B^{-1}=B^{-1}\# [\mathcal{A}^{\sfT} \mathcal{A}] (B) \\
			  & = B^{-1/2} (B^{1/2} [\mathcal{A}^{\sfT} \mathcal{A}] (B) B^{1/2})^{1/2} B^{-1/2} \\
			  & = B^{-1/2} ([\tilde{\mathcal{A}}^{\sfT} \tilde{\mathcal{A}}] (I) )^{1/2} B^{-1/2}.
		\end{aligned}
	\end{equation*}
	Furthermore, setting 
$$\tilde{Z} = B^{-1/2} Z B^{-1/2},$$ we get that 
	\begin{equation*}
		\begin{aligned}
			\langle Z, WZW \rangle ~=~ & \tr(ZWZW) \\
			~=~ & \tr(ZB^{-1/2} ([\tilde{\mathcal{A}}^{\sfT} \tilde{\mathcal{A}}] (I) )^{1/2} B^{-1/2}ZB^{-1/2} ([\tilde{\mathcal{A}}^{\sfT} \tilde{\mathcal{A}}] (I) )^{1/2} B^{-1/2}) \\
			~=~ & \tr(B^{-1/2}ZB^{-1/2} ([\tilde{\mathcal{A}}^{\sfT} \tilde{\mathcal{A}}] (I) )^{1/2} B^{-1/2}ZB^{-1/2} ([\tilde{\mathcal{A}}^{\sfT} \tilde{\mathcal{A}}] (I) )^{1/2} ) \\
			~=~ & \langle \tilde{Z}, ([\tilde{\mathcal{A}}^{\sfT} \tilde{\mathcal{A}}] (I) )^{1/2} \tilde{Z} ([\tilde{\mathcal{A}}^{\sfT} \tilde{\mathcal{A}}] (I) )^{1/2} \rangle. 
		\end{aligned}
	\end{equation*}
	Similarly
	\begin{equation*}
		\begin{aligned}
			\langle Z, [\mathcal{A}^{\sfT} \mathcal{A}] (Z) \rangle & = \langle B^{1/2} B^{-1/2} Z B^{-1/2} B^{1/2}, [\mathcal{A}^{\sfT} \mathcal{A}] (B^{1/2} B^{-1/2} Z B^{-1/2} B^{1/2}) \rangle \\
			& = \langle \tilde{Z} , B^{1/2}[\mathcal{A}^{\sfT} \mathcal{A}] (B^{1/2} \tilde{Z} B^{1/2}) B^{1/2} \rangle \\
			& = \langle \tilde{Z} , [\tilde{\mathcal{A}}^{\sfT} \tilde{\mathcal{A}}] (\tilde{Z}) \rangle.
		\end{aligned}
	\end{equation*}

To conclude the proof it remains to prove the theorem statement in the special case where $B=I$. Note that when $B=I$  we have 
$$W = [\mathcal{A}^{\sfT} \mathcal{A}] (I)\#I^{-1}=[\mathcal{A}^{\sfT} \mathcal{A}] (I)\#I=I\#[\mathcal{A}^{\sfT} \mathcal{A}] (I)=([\mathcal{A}^{\sfT} \mathcal{A}] (I))^{1/2},$$
where in the second to last equality we used that the geometric mean is symmetric in its two arguments and the least equality follows by the definition of the geometric mean \eqref{GM}.

Furthermore, by the definition  of the map $\cala$ we have that 
$$[\cala^\sfT\cala](Z)=\sum_{k=1}^m\la A_k,Z\ra A_k,$$
which in particular implies that  
%\begin{proposition} \label{thm:domination_identity}
%	Let $\mathcal{A} : \mathbb{S}^{n} \rightarrow \mathbb{R}^{d}$ be a linear map of the form
%	\begin{equation*}
%		\mathcal{A}(Z) = \left( \begin{array}{c}
%		\langle A_1,Z \rangle \\
%		\vdots \\
%		\langle A_d,Z \rangle
%		\end{array} \right),
%	\end{equation*}
%	where $A_1,\ldots,A_d$ are positive definite matrices.  Let $W = ([\mathcal{A}^{\sfT} \mathcal{A}] (I))^{1/2}$.  Then
%	\begin{equation*}
%		\langle Z, WZW \rangle \geq \langle Z, [\mathcal{A}^{\sfT} \mathcal{A}] (Z) \rangle 
%	\end{equation*}
%	for all $Z$.
%\end{proposition}
%\begin{proof}[Proof of Proposition \eqref{thm:domination_identity}] 
	$$W = ([\mathcal{A}^{\sfT} \mathcal{A}] (I))^{1/2} = \lp\sum_{k} \tr(A_k)  A_k\rp^{1/2}.$$
	Thus, in the case where $B=I$, the inequality we need to prove (cf. Equation \eqref{eq:main}) specializes to: 
			
			\be\label{main:inequality}
			\tr\lp Z \lp\sum_{k} \tr(A_k)  A_k\rp^{1/2} Z \lp\sum_{k} \tr(A_k)  A_k\rp^{1/2}\rp   \geq \sum_k \tr(A_kZ)^2,  \text{ for all } Z \in \mathbb{S}^{r}.
 \ee
As a special case of  Lieb's concavity theorem (e.g. see \cite[Theorem 6.1]{carlen}) we have that for any fixed real symmetric matrix $Z\in \bbS^n$, the real-valued map
$$(X,Y)\mapsto \tr(ZX^{1/2}ZY^{1/2})$$ 
is concave over  the domain  $\bbS^n_{++}\times \bbS^n_{++}$. In particular,  for any 
 $(X_1, Y_1), (X_2, Y_2)\in \bbS^n_{++}\times \bbS^n_{++}$ and $\lam \in [0,1]$ we have that  
 $$\tr(Z(\lam X_1+(1-\lam)X_2)^{1/2}Z(\lam Y_1+(1-\lam)Y_2)^{1/2})\ge \lam \tr(ZX_1^{1/2}ZY_1^{1/2})+  (1-\lam) \tr(ZX_2^{1/2}ZY_2^{1/2}).$$
 In turn, setting $X_1=Y_1={\tr(A_1)\over \lam}A_1$ and $X_2=Y_2={\tr(A_2)\over 1-\lam}A_2$  we get that:
  $$
  \begin{aligned}
  &\tr(Z(\tr(A_1)A_1+\tr(A_2)A_2)^{1/2}Z(\tr(A_1) A_1+\tr(A_2)A_2)^{1/2})\ge \\
  &\tr(A_1) \tr(ZA_1^{1/2}ZA_1^{1/2})+   \tr(A_2)\tr(ZA_2^{1/2}ZA_2^{1/2}). 
  \end{aligned}
  $$
  Finally, by induction it follows that:
   \begin{equation}\label{sdvsvbs}
   \tr\lp Z(\sum_k \tr(A_k)A_k)^{1/2}Z( \sum_k (\tr(A_k)A_k)^{1/2}\rp \ge \sum_k \tr(A_k) \tr(ZA_k^{1/2}ZA_k^{1/2}),
   \end{equation}
  for any family of positive definite matrices $A_1, \ldots, A_m$ and any fixed matrix $Z$. 
    Based on \eqref{sdvsvbs}, to prove   \eqref{main:inequality} it remains to show that
    
    \be\label{cdvd}    \sum_k \tr(A_k) \tr(ZA_k^{1/2}ZA_k^{1/2})\ge \sum_k \tr(A_kZ)^2. 
    \ee
    We prove  inequality \eqref{cdvd} term-by-term, i.e., we show that 
        \be\label{cdsvds}
         \tr(A_k) \tr(ZA_k^{1/2}ZA_k^{1/2})=\tr(A_k)\tr((ZA_k^{1/2})^2)\ge  \tr(A_kZ)^2. 
         \ee
        	For this we use that for any  $X,Y \in \mathbb{S}^{n}$ we have 
	\begin{equation}\label{csvsd}
		\tr(XY)^2
		 \leq \tr(X^2) \cdot \tr(Y^2). 
	\end{equation}
Indeed,  let  $\sigma_1 \leq \ldots \leq \sigma_n$ be the singular values of $X$ and $\mu_1 \leq \ldots \leq \mu_n$ be the singular values of $Y$.  Then
\begin{equation*}
	\tr(XY)^2 \leq \left( \sum_{i=1}^{ n} \sigma_i \mu_i \right)^2 \leq \left( \sum_{i=1}^{n} \sigma_i^2 \right) \left( \sum_{i=1}^{n} \mu_i^2 \right) = \tr(X^2) \cdot \tr(Y^2).
\end{equation*}
The first inequality follows from the von Neumann's trace inequality (see e.g. \cite{bhatia}) and the second inequality follows from the Cauchy-Schwarz inequality.

Lastly, by \eqref{csvsd} we have that 
$$\tr(A_kZ)^2=\tr(A_k^{1/2}(A_k^{1/2}Z))\le \tr(A_k)\tr((ZA_k^{1/2})^2),$$
which is exactly 
\eqref{cdsvds}.
\end{proof}

\section{Fixed-points of the MWU algorithm are KKT points}
In this section we give the proof of Theorem \ref{fixedpointsthm}. 

\begin{lemma} \label{thm:kkt_actualresult} Let $\mathcal{A}$ be the linear map $\mathcal{A}(Z) = (\mathrm{tr}(A_1 Z), \ldots, \mathrm{tr}(A_m Z))^\sfT$, where $A_i$ are positive definite matrices, and let $x$ be a vector with positive entries.  Suppose $B$ is a positive definite matrix satisfying $B =W (\mathcal{A}^\top x) W$, where $W = ([\mathcal{A}^{\sfT} \mathcal{A}] (B))^{-1}\#B$.  Then $\cala^\sfT x =[\cala^\sfT \cala] (B)$.
\end{lemma}

\begin{proof}  Since $B$ is positive definite, it follows that $[\mathcal{A}^{\sfT} \mathcal{A}] (B)=\sum_{i=1}^m\la A_i,B\ra A_i$ is also positive definite, and thus $W = ([\mathcal{A}^{\sfT} \mathcal{A}] (B))^{-1}\#B$ is positive definite.  We then have that
$$\mathcal{A}^\top x=W^{-1}BW^{-1}=(B^{-1}\#[\mathcal{A}^{\sfT} \mathcal{A}] (B))B(B^{-1}\#[\mathcal{A}^{\sfT} \mathcal{A}](B))=[\mathcal{A}^{\sfT} \mathcal{A}](B),$$
where 
the last equality follows by the unicity property of the matrix geometric mean \eqref{riccati}.
\end{proof}

==> manuscript PSD case: arxiv/sec_existing.tex <==
\section{Prior works on computing PSD factorizations}
All 
existing algorithms for computing PSD factorizations  employ the alternating minimization approach described in the previous section, where we fix one set of variables and minimize over the other, and essentially boil  down into finding algorithms for  the convex problem \eqref{main}.

% In the following, we discuss prior works for minimizing \eqref{bigboss} by focusing on the following sub-problem:
%\be\label{small}
%\inf \Big\{\|x-\mathcal{A}(B)\|^2: \  B \in \psd^r  \Big\}.
%\ee

\paragraph{Projected Gradient Method (PGM).}  The first approach for computing PSD factorizations  is based on  applying PGM to \eqref{main}, alternating  between a gradient step to minimize the objective and  a projection step onto the set of PSD matrices \cite{VGG18}.  The latter projection step uses the following useful fact: Given the spectral decomposition $C=U{\rm diag}(\lam_i)U^\sfT$ of a matrix $C\in \bbS^n$, the projection onto the PSD cone is $U{\rm diag}(\max(0,\lam_i))U^\sfT$ \cite{hig}.  The vanilla PGM has slow convergence rate, so the authors in \cite{VGG18} also propose an accelerated variant that incorporates a momentum term.

\paragraph{Coordinate Descent.}  The authors in \cite{VGG18} also propose a different algorithm combining the ideas of coordinate descent and  a change of variables that allows them to also control  the rank of the PSD factors, which  was popularized by  the seminal work of Burer and Monteiro for solving rank-constrained SDPs \cite{BM}. 
%explicitly expressing each factor in its PSD factorization to enforce the PSD constraint. 
  Concretely, the authors use the  parameterization  $A_i=a_ia_i^\sfT$, and $B_j=b_jb_j^\sfT$, where $a_i\in \R^{r\times r_{A_i}}$, and $b_j\in \R^{r\times r_{B_j}}$ for some fixed $r_{A_i}, r_{B_j}\in \mathbb{N}$, and optimize using a coordinate descent scheme over  the entries of the matrices $a_i$ and $b_j$.
  %  This approach is frequently associated  with  the seminal work of Burer and Monteiro for solving rank-constrained SDPs \cite{BM}, and has the advantage that the matrices $A_i$ and $B_j$ may be rank deficient. %The BM approach relies on the observation that  an  $n$-by-$n$ psd matrix $X$ with rank $r$ can be written as $X=\sum_{i=1}^rx_ix_i^\sfT=XXT$ for some real vectors $x_1,\ldots, x_r\in \R^{n\times 1}$. 
%Specifically, fixing (in some ad-hoc manner) the ranks $r_{A_i}$ and $r_{B_j}$ for each $A_i$ and $B_j$ respectively, it follows that there exists matrices $a_i\in \R^{r\times r_{A_i}}$ and  $b_j\in \R^{r\times r_{B_j}}$ such that  $A_i=a_ia_i^\sfT$ and $B_j=b_j{b_j}^\sfT$.  
Thus,  problem \eqref{main}~becomes: 
\be\label{BM}
 \underset{b}{ \inf} ~~ \| x - \mathcal{A} (bb^\sfT) \|_2^2 \quad \mathrm{s.t.} \quad  b\in \R^{r\times r_B},
 \ee
which is a quartic polynomial in the entries of $b$.  Thus, its gradient is a cubic polynomial, 
%as the following problem over the $a_i$'s and $b_j$'s:
%\be\label{factorformulation}
%{\inf} \Big\{ \sum_{i,j}(X_{ij}-a_i^\sfT b_j)^2: \ a_i\in \R^{r\times r_{A_i}},  b_j\in \R^{r\times r_{B_j}}\Big\}.
%\ee 
%The algorithm proceeds by fixing one set of variables -- say the $a_i$'s -- while updating the other set -- say the $b_j$'s.  The resulting problem entails the minimization of a degree four polynomial over $\R_+$, 
and its roots can be found  using  Cardano's method (and careful book-keeping). %an explicit formula for  the roots of a cubic polynomial (as Cardano's method).
 
% We conclude with a note on the convergence properties of the coordinate descent method: Every limit point of the sequence of iterates generated by the CD method is a stationary  point if the minimum in each CD subproblem is uniquely attained (assuming a convex objective function and convex constraint sets) \cite{Ber}.  Nevertheless, note that these assumptions are not necessarily satisfied in this case.   Lastly, we note that  an additional desirable  feature of the factor-based formulation~(\eqref{factorformulation}) is that   it allows to explicitly  control the rank  of the PSD factors, i.e., the $r_j$'s. 


\paragraph{Connections to Affine Rank Minimization and Phase Retrieval.}  A different set of algorithms developed in \cite{LF20, LF20b, LLTF20} is based on the connections between computing PSD factorizations with the affine rank minimization (ARM) and the phase retrieval (PR) in signal procesing.  
First, recall that the PSD-ARM problem focuses on  recovering a low-rank matrix from affine measurements:
$$
 \min_B ~~ \rank(B) \quad \text{s.t.} \quad   \ \cala(B)=x, \ B\in \psd^r.
$$
Here, $\cala$ is a known linear map representing measurements while $x$ is known vector of observations. Due to the non-convexity of the rank function, a useful heuristic initially popularized in the control community  is to replace the rank by  the trace function, e.g., see \cite{MP} and \cite{fazel}, in which case the resulting problem is an instance of an SDP.  A different  heuristic for   PSD-ARM is to find a PSD matrix of rank at most $k$ that  minimizes the squared loss function, i.e., \be\label{cdsfvsdfv}
 \inf~~ \|x-\cala(B)\|_2^2 \quad \text{s.t.} \quad  B\in \psd^r, \ \rank(B)\le k,
\ee
where alternatively, the rank constraint can be enforced  by parametrizing the PSD matrix variable $B\in \psd^r$ as $B=bb^\sfT$ with $b\in \R^{r\times k}$. 
The point of departure for the works  \cite{LF20, LLTF20, LF20b} is that problem~\eqref{cdsfvsdfv}  corresponds exactly to  the sub-problem \eqref{main} encountered in any alternate minimization strategy for computing  PSD factorizations,   albeit with an additional  rank constraint. In view of this, any  algorithm  from the signal processing literature developed for ARM can be applied to \eqref{main}.


%can be optimized using existing methods in the literature that were developed for phase retrieval and ARM.

The main algorithms considered in \cite{LF20, LF20b, LLTF20}  are Singular Value Projection (SVP)  \cite{SVP},   Procrustes Flow \cite{procrsustes}, and variants thereof.
%which  involves an initialization phase   based on SVP  followed by a  second phase which  essentially performs gradient descent with a meticulously  chosen step size. 
In terms of convergence guarantees,  for affine maps $\mathcal{A}$  obeying the  Restricted Isometry Property \cite{RIP}, both algorithms converge to an optimal solution. Nevertheless, it is unclear whether these guarantees carry over when applied to the PSD factorization problem. 

%The link to the phase retrieval problem becomes apparent when   we restrict to   PSD factorizations with rank-1 factors,  i.e., $A_i=a_ia_i^\sfT$ and $B_j=b_jb_j^\sfT$, for some $r$-dimensional vectors $a_i, b_j$. In this setting, a PSD factorization of the data matrix $X$ can be interpreted as:
%$$X_{ij}\approx \mathrm{tr}( A_i B_j )=|\la a_i,b_j\ra|^2.$$
%Assuming as usual that  the $a_i$'s are fixed,   this is just the problem  of recovering a signal (the $j$-th column of $X$)  from phaseless
%measurements  given by the sensing vectors $a_1, \ldots, a_m$. 



%Lastly, note   that \eqref{small} is an instance of a convex quadratic semidefinite program, i.e., an optimization problem of the form:
%$$
%\min \{{1\over 2} \la X, \mathcal{Q}(X)\ra+\la C,X\ra:\ \mathcal{L}(X)=b, X\succeq 0 \},$$
%where $\mathcal{Q}: \mcs^n\to \mcs^n$  is a self-adjoint positive semidefinite linear operator on  (i.e., $\la X, \mathcal{Q}(X)\ra\ge~0, \forall X\in \mathcal{S}^n$), $b$ is a vector in $\R^m$ and $\mathcal{L}$ a linear mapping from $\mcs^n\to \R^m$. Indeed, in this case we have that $\mathcal{Q}=\cala\cala^\sfT$ which is psd as 
%$\la X, \mathcal{Q}(X)\ra=\|\cala(X)\|_F^2\ge0$.
%



==> manuscript PSD case: arxiv/sec_framework_CURRENT.tex <==
\section{A Matrix Multiplicative Update  Algorithm for  PSD Factorizations}\label{sec2}

%[State algorithm]
In this section we describe our algorithm for computing (approximate) PSD factorizations of a matrix $X$. As already discussed, we employ an alternate optimization approach where we alternate between optimizing with respect to the $A_i$'s and the $B_j$'s. 
The sub-problem in each update step symmetric in the variables $A_i$ and $B_j$, with the small modification where we replace $X$ with its transpose.  As such, in the remainder of this discussion, we assume without loss of generality that   the $A_i$'s are fixed and we update the $B_j$'s. The resulting sub-problem we need to solve is \eqref{main}.

%[This is an instance of a MM-algorithm, What briefly is an MM-algorithm, what you get out of it]

\paragraph{Majorization-Minimization (MM) Framework.}  Our algorithm is an instance of the (MM) framework, e.g. see \cite{Lange} and references therein. To briefly describe this approach, suppose   we need to solve the optimization problem  $\min \{F(x): x\in \mathcal{X}\}.$  
The MM framework  relies on the existence of a parametrized family of  auxilliary functions  $u_x: \mathcal{X}\to \R$, one for each $x\in \mathcal{X}$,~where:
\be\label{auxilliary}
 F(y)\le u_x(y),  \ \text{for all } y\in \mathcal{X}\  \text{ and } \ F(x)=u_x(x).
 \ee
%\item ${\rm argmin} \{ u_x: x\in {\rm dom}(f)\}$ is easy to find. 
Based on these two properties,  $F$ is nonincresasing under the  update rule:
 \be\label{updaterule}
  x^{\new} =\amin \{ u_{x^{\old}}(y):\ y \in \mathcal{X}\},
  \ee
as can be easily seen by the following chain of inequalities
$$f(x^{\new})\le u_{x^{\old}}(x^{\new})\le u_{x^{\old}}(x^{\old})=f(x^{\old}).$$

We conclude with two important remarks concerning  the MM framework. First, note that although the iterates generated by the MM  update rule  \eqref{updaterule} are nonincreasing  in objective function value, there is in general no guarantee that they converge to a minimizer. Secondly,  for the MM approach to be of any use, the auxilliary functions employed at each iteration need to be easy to~optimize. 





%$\min \{f(A,B): A,B\in \mathcal{X}_A\times \mcx_B\}$ -- see~\cite{Lange} and references therein.  The MM method entails finding a parametrized family of  auxilliary functions $u_{A} (\cdot,B)$ and $u_{B} (A,\cdot)$ that satisfy the following properties:
%\be\label{domination}
%\bal
%f(\cdot, B)\le u_A(\cdot, B)  \ \forall A,B &  \quad\text{ and } \quad f(A,B)=u_A(A,B) \\ 
%f(A,\cdot)\le u_B(A, \cdot) \ \forall A,B& \quad\text{ and } \quad  f(A,B)=u_B(A,B)
%\eal 
%\ee
%Suppose we perform updates on the variables $A$ and $B$ as follows:
%\be\label{MMupdate} 
%\bal 
%\an& =\amin \{ u_{\ao}(A, \bo): \ A \in \mcx_A\}, \\
%\bn&=\amin \{ u_{\bo}(\an, B):\ B\in \mcx_B\}.
%\eal
%\ee
%Then $f(\ao,\bo)=u_{\ao}(\ao,\bo) \ge u_{\ao}(\an,\bo) \ge f(\an,\bo)=u_{\bo}(\an,\bo)\ge u_{\bo}(\an,\bn)\ge f(\an,\bn)$; i.e., the function $f$ is non-increasing under the update rule \eqref{MMupdate}.  In particular, the MM method is most effective if we identify a suitable family of auxilliary functions such that (i) the associated update step in \eqref{MMupdate} is simple to compute, and (ii) the method makes a reasonable amount of progress in each iteration.

\paragraph{Matrix Geometric Mean.}  Our choice of auxilliary functions relies  on the well-studied  notion of a geometric mean between a pair  of positive definite matrices, whose definition  we recall next. For additional details and omitted proofs  the reader is referred to  \cite{gmeam} and \cite{bhatia}.
  The matrix geometric mean of  two positive definite matrices $C$ and $D$ is given by %the  expression:
\begin{equation}\label{GM}
	C\# D= C^{1/2} (C^{-1/2} D C^{-1/2})^{1/2} C^{1/2},
\end{equation}
or equivalently, it is the unique positive definite solution of the Riccati equation 
\be\label{riccati}
XC^{-1}X=D,
\ee in the matrix variable $X$. The matrix geometric mean also has a nice geometric interpretation in terms of  the Riemannian geometry     of the manifold of  positive definite matrices, and specifically, $C\# D$   is the midpoint of the unique geodesic joining $C$ and $D$. 
Finally, the  matrix geometric mean is symmetric in its two arguments  $C \# D = D \# C$ and also satisfies $(C\#D)^{-1} = C^{-1} \# D^{-1}$. 

\paragraph{The MMU Algorithm for PSD Factorizations.}  The main step for deriving our algorithm for approximately computing PSD factorizations is to apply  the MM framework, with a meticulously chosen   auxilliary function,  to the convex quadratic SDP~\eqref{main}. Our main result is the following:
%$$
% \underset{B}{ \inf} ~~ \| x - \mathcal{A} (B) \|_2^2 \quad \mathrm{s.t.} \quad  B \in \psd^r,
%$$

\begin{theorem}\label{LSstylethm}
Consider a fixed vector  $x\in \R^m_+$  and let
$\mathcal{A} : \mathbb{S}^{r} \rightarrow \mathbb{R}^{m}$ be the linear map defined by
$Z\mapsto \mathcal{A}(Z) = \left( \tr (A_1Z), \ \ldots \  ,\tr( A_mZ) \right),$
for some fixed $r \times r$ positive definite  matrices $A_1,\ldots, A_m$. Then, the objective function 
$\| x - \mathcal{A} (B) \|_2^2$ is non-increasing under the update rule
$$\bn = W(\mathcal{A}^\top x) W, \quad \text{where} \quad W= ([\mathcal{A}^{\sfT} \mathcal{A}] (\bo))^{-1}\#(\bo),$$
and moreover, if  initialized with a positive definite matrix, the iterates remain positive definite. 
\end{theorem}

\begin{proof}First, note that if the $A_i$'s and $\bo$ are all  positive definite, the  update rule is well-defined. Indeed, we have    $ [\mathcal{A}^{\sfT} \mathcal{A}] (\bo)=\sum_{k=1}^m\tr( A_k\bo) A_k$ is also positive definite, and thus invertible.

Set $F(B):=\| x - \mathcal{A} (B) \|_2^2$ and define the function
\begin{equation} \label{eq:auxilliary}
u_{\bo}(B) := F(\bo)+\la \nabla F(\bo), B-\bo\ra+\la B-\bo, T(B-\bo)),
\end{equation}
where $T: \mathbb{S}^r\to \mathbb{S}^r$ is the operator given  by
\begin{equation*}
T(Z) = W^{-1}ZW^{-1} \quad \text{ and } \quad W= ([\mathcal{A}^{\sfT} \mathcal{A}] (\bo))^{-1}\#(\bo).
\end{equation*}
The claim of the theorem will follow  as an immediate consequence of the MM framework, as long as we establish  that $u_{\bo}(B)$ is an auxilliary function, i.e., it satisfies the two properties given in~\eqref{auxilliary}. 

Clearly, we have that $u_{\bo}(\bo)=F(\bo)$, so it only remains to show the domination property, that is,  
 $u_{\bo}(B)\le F(B), $ for all $B\in \psd^r$.  In fact, we show a slightly stronger result, namely that  $u_{\bo}(B)\le F(B)$ holds  for all symmetric  matrices $B\in \mathbb{S}^r$.  To see this we use the second order Taylor expansion of $F$ at $\bo$, which  as $F$ is quadratic in $B$,  is given by
\begin{equation}\label{eq:taylor}
F(B)=F(\bo)+\la \nabla F(\bo), B-\bo\ra+\|\mca(B-\bo)\|_2^2.
\end{equation}
Comparing the expressions \eqref{eq:auxilliary} and \eqref{eq:taylor}, to show that $F(B)\le u_{\bo}( B)$ for all $B\in \mathbb{S}^r$ it suffices to check that the operator $T - \mathcal{A}^{\sfT} \mathcal{A}$ is positive; i.e., $\langle Z, [T - \mathcal{A}^{\sfT} \mathcal{A}] (Z) \rangle \ge 0$ for any matrix $Z\in \mathbb{S}^r$. 
This claim is the main technical part of the proof,  deferred to Lemma \ref{thm:domination_general} in  the Appendix. 


Furthermore, the fact that $T - \mathcal{A}^{\sfT} \mathcal{A}$ is a positive operator, also implies that $T$ is itself   a positive operator. Consequently,  the MM update  \eqref{updaterule} obtained  by using   the auxilliary function \eqref{eq:auxilliary} can be calculated just by setting the gradient equal to zero, and is given by
\begin{equation} \label{eq:psd_update1}
B_{\mathrm{new}} = B_{\mathrm{old}} - T^{-1} \left( [\mathcal{A}^{\sfT} \mathcal{A}] (B_{\mathrm{old}}) - \mathcal{A}^{\sfT}(x) \right).
\end{equation}
Moreover, as $T^{-1} (Z) = W Z W$ and $W= ([\mathcal{A}^{\sfT} \mathcal{A}] (\bo))^{-1}\#(\bo)$ it follows that 
\be\label{cdsvs}
B_{\mathrm{old}} =W ([\mathcal{A}^{\sfT} \mathcal{A}] (B_{\mathrm{old}}))W= T^{-1} ( [\mathcal{A}^{\sfT} \mathcal{A}] (B_{\mathrm{old}})),
\ee
where for the first equality we use the unicity property of the matrix geometric mean (recall \eqref{riccati}). 
Subsequently, using \eqref{cdsvs}, the MM update rule in~\eqref{eq:psd_update1} simplifies to the following:
\be\label{updatenew}
B_{\mathrm{new}} = T^{-1}(\mathcal{A}^\sfT \bx)=W(\mathcal{A}^\sfT \bx)W.
\ee

Lastly, since the  $A_i$'s are PSD, it follows that $\cala^\sfT \bx=\sum_i x_i A_i$ is a conic combination of PSD matrices (recall that $x\in \R^m_+$), and thus, it is itself PSD.   Consequently,  $B_{\mathrm{new}}$ is PSD.   In fact, if the matrices $A_i$ and $B_{\mathrm{old}}$ are positive definite,  the updated matrix $B_{\mathrm{new}}$ is also  positive definite.
\end{proof}

%
%
%\begin{theorem} \label{thm:domination_general}
%Let $\{A_1,\ldots,A_m\}$ be a collection of positive definite matrices and let $\mathcal{A}$ be the linear mapping defined by
%\begin{equation*}
%\mathcal{A} : \mathbb{S}^{r} \rightarrow \mathbb{R}^{m} \text{ where } Z\mapsto \left(
%\mathrm{tr}(A_1 Z), \ \ldots \ 
%,\mathrm{tr}(A_m Z) \right)^\sfT.
%\end{equation*}
%Suppose $B \in \mathbb{S}^{r}$ is positive definite.  Let 
%$$W = [\mathcal{A}^{\sfT} \mathcal{A}] (B)\#B^{-1}.$$ 
%Then
%\begin{equation}\label{eq:main}
%\langle Z, WZW \rangle \geq \langle Z, [\mathcal{A}^{\sfT} \mathcal{A}] (Z) \rangle \quad  \text{ for all } \quad Z \in \mathbb{S}^{r}.
%\end{equation}
%\end{theorem}

%Third, the note that the update rule only requires the computation of the geometric mean of two matrices as a primitive -- this can be achieved, for instance, by computing the spectral decomposition of these matrices.
Having established an iterative method  for problem \eqref{main} that is non-increasing in value and retains PSDness, we can  incorporate  this as a sub-routine  in our alternating optimization scheme  for computing  PSD factorizations. 
The pseudocode  of the resulting method is given in Algorithm~\ref{alg}.


%\begin{algorithm}{MM Algorithm for Computing PSD Factorizations }[]{} 
%\qinput{A matrix $X\in \R^{m\times n}_{\ge 0}$, parameter $r\in \mathbb{N}$} 
%\qoutput{ $\{ A_1,\ldots, A_m \},\{ B_1, \ldots, B_n \} \subseteq \bbS^r_+$, $X_{ij}\approx \tr(A_iB_j)$ for all $i,j$}
%while stopping criterion not satisfied: \\
% \be\label{updaterule}
%  \bal 
%A_i & \leftarrow V_i (\mcb^\top x_i) V_i \quad \text{ where } \quad V_i =([\mcb^{\sfT} \mcb] (A_i))^{-1}\# A_i, \quad x_i = X_{ i : }  \\
%B_j & \leftarrow W_j (\mathcal{A}^\top x_j) W_j \quad \text{ where } \quad W_j = ([\mathcal{A}^{\sfT} \mathcal{A}] (B_j))^{-1}\#(B_j), \ x_j = X_{: j}
%\eal 
%\ee
%     \end{algorithm}

%
\begin{algorithm}[h]
  \caption{ Matrix Multiplicative  algorithm for  computing PSD factorizations}
   \textbf{Input:} A matrix $X\in \R^{m\times n}_{\ge 0}$, parameter $r\in \mathbb{N}$\\
  \textbf{Output:}    $\{ A_1,\ldots, A_m \},\{ B_1, \ldots, B_n \} \subseteq \bbS^r_+$, $X_{ij}\approx \tr(A_iB_j)$ for all $i,j$
 \begin{algorithmic}\label{alg}
  \STATE while stopping criterion not satisfied: 
  \STATE 
  \be\label{updaterule}
  \bal 
A_i & \leftarrow V_i (\mcb^\top x_i) V_i \quad \text{ where } \quad V_i =([\mcb^{\sfT} \mcb] (A_i))^{-1}\# A_i, \quad x_i = X_{ i : }  \\
B_j & \leftarrow W_j (\mathcal{A}^\top x_j) W_j \quad \text{ where } \quad W_j = ([\mathcal{A}^{\sfT} \mathcal{A}] (B_j))^{-1}\#(B_j), \ x_j = X_{: j}
\eal 
\ee
\end{algorithmic}
\end{algorithm}

\if0
Note that by \eqref{PDmatrix} the matrix $[\mathcal{A}^{\sfT} \mathcal{A}] (B_{\mathrm{old}})$ is positive definite, so considering its geometric  mean with the positive definite  matrix $\bo^{-1}$ indeed makes sense. 
Furthermore, condition $(ii)$ is satisfied as the Hessian of the function $\la B, T(B)\ra=\tr(BQBQ)$ is equal to $Q\otimes Q$, which is positive definite as the geometric mean is (by definition) positive definite, and the tensor product of positive definite  matrices is also positive definite. 



We conclude with some   general remarks concerning various algorithmic aspects of the MM framework. First, in terms of  its convergence properties,  the fact that  the iterates generated by the MM  algorithm are nonincreasing  in objective function value (which is lower bounded by zero), shows that the sequence of values  $(f(A_k,B_k))_k$ converges.  %With mild additional assumptions  it is also true that any limit point of the sequence $(f(A_k,B_k))_k$ is a KKT point of (\eqref{bigboss}), e.g., see \cite{}
Secondly,  for the MM approach to be of any use, the optimization problems  \eqref{MMupdate}  encountered at each iterationneed to be tractable. Third, note that the  update rule  given in \eqref{MMupdate}  is not amenable to parallel implementation  with respect to the $A$'s and the $B$'s, as the update rule for $B$ depends on $\an$. The similar problem is also present in Lee-Seung's original algorithm for NMF, but a new approach  for NMF where the updates can be made concurrently was recently given in~\cite{PSVW}. 

%Using this notaion , our problem 
%This problem is minimized in an ietrative manner, first with 
%We repeat the same procedure for PSD factorization.where $A_1,\ldots,A_d$ are positive definite matrices.  Let $B \in \mathbb{S}^{n}$ be positive definite.  The matrix $B$ represents our current estimate to the equation
%\begin{equation*}
%	\mathcal{A} (B) \approx \bx.
%\end{equation*}
%Our goal is to develop an analogous update procedure.

In this work we   use  the MM approapch  to solve the optimization problem \eqref{main}, where for  simplicity of presentation we assume that $A_1, \ldots, A_n$ are fixed and  focus on the $B$'s. Our goal  is to  
minimize $f(A,B)={1\over 2}\sum_i(X_{ij}-\tr(A_iB))^2$, where the matrix variable $B$  is an  $r$-by-$r$ PSD matrix.   To simplify notation, we omit the dependency on the $A$'s (as they are fixed),  and define
$$f(A,B )=F(B).$$ 
  The first step is to find an appropriate family of auxilliary functions. As our objective function
 is a quadratic in $B$,  the second order Taylor expansion at $\bo$ is a tautology, specifically: 
$$F(B)=F(\bo)+\la \nabla F(\bo), B-\bo\ra+\|\mca(B-\bo)\|_F^2,$$
%\la B-\bo,  [\mca^\sfT \mca](B-\bo)),$$
where the transpose of the mapping $\mca$ is given by:
\be
\mathcal{A}^\sfT: \R^m\to \mathbb{S}^r \quad x\mapsto \sum_{i=1}^mx_iA_i.
\ee 
Consequently,  for any invertible linear map $T: \mathbb{S}^r\to \mathbb{S}^r$ satisfying  the following two properties:
\begin{itemize}
\item[$(i)$]  $T-\mathcal{A}^{\sfT} \mathcal{A}:  \mathbb{S}^r\to \mathbb{S}^r$  is a positive operator% i.e., $\langle Z, [\mathcal{A}^{\sfT} \mathcal{A}] (Z) \rangle \leq  \langle Z, T(Z) \rangle $ 
%	for all $Z \in \mathbb{S}^{r}$.
\item[$(ii)$] $T: \mathbb{S}^r\to \mathbb{S}^r$ is a positive operator.
%The function ${1\over 2}\|x\|^2-2\la \mathcal{A}^\sfT(x),B\ra + \langle B, T(B) \rangle$ is convex,
\end{itemize}
\fi
 

==> manuscript PSD case: arxiv/sec_intro_CURRENT.tex <==
\section{Introduction}

Let $X\in \R_+^{m\times n}$ be a $m \times n$ dimensional matrix with non-negative entries and  $r\in~\mathbb{N}$ a user-specified parameter.  
An {\em $r$-dimensional  positive semidefinite (PSD) factorization} of $X$ is given  by two families  of 
  $r\times r$  PSD matrices $A_1,\ldots, A_m$ and $B_1,\ldots,B_n$  satisfying 
\be\label{factorization}
X_{ij}= \tr(A_iB_j),\   i\in [m],\ j\in [n].
\ee
  %We refer to the   problem of finding a PSD factorization  as the  {\em PSD factorization  problem}. 
%
%We say that $X$ admits a {\em positive semidefinite (PSD) factorization} of rank $r$ if there exists a collection of $r\times r$-dimensional PSD matrices $\{A_1,\ldots, A_m\}$ and $\{ B_1,\ldots,B_n \}$ satisfying:
%\be\label{factorization}
%X_{ij}=  \tr(A_iB_j), \quad  i\in [m],\ j\in [n].
%\ee
%%We refer to the process of deriving the collection of matrices $\{A_1,\ldots, A_m\}$ and $\{ B_1,\ldots,B_n \}$ as computing an \emph{exact rank-}$r$ {\em PSD factorization} of $X$.
%Quite frequently, we are also interested in computing an \emph{approximate} PSD factorization in which we fix the parameter $r$, and we compute a PSD factorization of rank $r$ that best approximates $X$, say, with respect to the squared loss:
%\be\label{bigboss}
%\inf \bigg\{\sum_{i,j}(X_{ij}-\mathrm{tr}(A_i B_j))^2: \ A_i, B_j\in \psd^r  \bigg\}.
%\ee
Every non-negative matrix admits an $r$-dimensional PSD factorization for an appropriate value of~$r\in\mathbb{N}$--we may, for instance, take $A_i={\rm diag}(X_{i:})$ and $B_j={\rm diag}(e_j)$, a choice that corresponds to  an $n$-dimensional PSD factorization.  The smallest $r\in \mathbb{N}$ for which $X$ admits an $r$-dimensional  PSD factorization is called   the \emph{PSD-rank} \cite{psdrank}.

%Consider a  data matrix   $X\in \R_+^{m\times n}$   with nonnegative entries and a user-specified parameter $r\in~\mathbb{N}$. An $r$-dimensional {\em positive semidefinite (PSD) factorization} of $X$ is specified by two families  of 
%  $r\times r$  PSD matrices $A_1,\ldots, A_m$ and $B_1,\ldots,B_n$  satisfying 
%\be\label{factorization}
%X_{ij}= \tr(A_iB_j),\   i\in [m],\ j\in [n],
%\ee
%  We refer to the   problem of finding a PSD factorization of some fixed size $r$  as the  {\em PSD factorization  problem}. 
%Note that  an entrywise nonnegative  matrix  $X\in \R_+^{m\times n}$ always admits a PSD factorization for an appropriate value of $r$, e.g., taking   $A_i={\rm diag}(X_{:i})$ and $B_j={\rm diag}(e_j)$ gives     a  PSD factorization of $X$ of size $n$. The smallest possible  $r\in \mathbb{N}$ for which  $X\in \R_+^{m\times n}$ admits a PSD factorization with $r\times r$ PSD matrices  is called the positive semidefinite rank (PSD-rank) of $X$ \cite{psdrank}. %In this setting, the matrices $A_i$ and $B_j$ are called the PSD factors and $r$ is the size of the factorization. 

 PSD factorizations are of fundamental importance   to a wide  range of areas, most notably
 towards  understanding  the  expressive power  of linear optimization over the cone of  positive semidefinite matrices,   \cite{lifts, sam}, 
 studying  the power and  limitations of quantum resources within the framework  of information theory \cite{qcorr,sam}, and  as a natural non-commutative generalization of the  extremely popular dimensionality reduction technique  of    non-negative matrix factorizations (NMFs) \cite{PT, Lsnature, LS00}. We elaborate further on the relevance of PSD factorizations to each of these areas~below. 
 


%
%PSD factorizations generalize non-negative matrix factorizations (NMFs) \cite{Lsnature,LS00} -- if we take each of the matrices $A_i$ and $B_j$ \eqref{factorization} to be diagonal, then we recover a NMF.  PSD factorizations are fundamental in a range of application areas such as understanding the expressive power of semidefinite programs \cite{sam,lifts} as well as understanding the power and limitations of quantum resources within the framework  of information theory \cite{sam,qcorr}.
%%The importance of the  PSD factorization problem   is  motivated  by  its     relevance   to a wide  range of areas, most notably
%% towards  understanding  the  expressive power  of linear optimization over the cone of  positive semidefinite matrices  \cite{lifts, sam}, 
%% understanding the power and  limitations of quantum resources within the framework  of information theory \cite{qcorr,sam}, and  as a natural non-commutative generalization of the  extremely popular dimensionality reduction technique  of    nonnegative matrix factorizations (NMFs) \cite{Lsnature, LS00}. 
%We elaborate on these connections in the following.
%We elaborate further on the relevance of PSD factorizations to each of these areas below. 
 
\paragraph{Links to Semidefinite Programming.}  A Semidefinite Program (SDP) is a convex optimization problem  in which we minimize a linear function over the set of PSD matrices intersected with an affine subspace.  SDPs are a powerful generalization of Linear Programs
with extensive modeling power and tractable algorithms for solving them, e.g., see \cite{sdp} and references therein.  SDPs are frequently used as convex relaxations to combinatorial problems, and have many important applications   including   optimal power flow computation  \cite{lavaei}, robustness certification to adversarial examples in neural networks \cite{adversarial}, and inference in graphical models \cite{inference}. 
% A semidefinite program (SDP)  corresponds to optimizing a linear function over an affine slice of the cone of positive semidefinite matrices. SDPs are an extremely useful family of optimization problems with extensive modeling power and tractable algorithms for solving them, e.g. see \cite{sdp}. Applications of SDPs abound, some notable examples being the optimal power flow problem \cite{lavaei},   robustness certification  to adversarial examples in neural networks  \cite{adversarial}+ ADD more  data science applications 

 Given a bounded  polytope $P = \{x\in \R^d: c_i^\sfT x\le d_i, \ i\in [\ell]\}={\rm conv}(v_1,..,v_k)$,  a basic question concerning  the expressive power of SDPs is  to find  the \emph{smallest} possible SDP description of $P$, i.e.,  
 the minimum $r\in \mathbb{N}$ for which we can express $P$ as the projection of an the affine slice %
 of the cone of $r\times r$  PSD matrices. Concretely, the goal in this setting  is  to express $P$ as:
%of the collection of $r \times r$ PSD matrices:
\be\label{psdlift}
P=\pi(\psd^r \cap \mathcal{L}),
\ee
where $\psd^r $ is the cone of  $r\times r$  PSD matrices, $ \mathcal{L}$ is an affine subspace of the space of $r\times r$ symmetric matrices and $\pi$ a linear projection from the space of $r\times r$ symmetric matrices to $\R^d$.   A representation  of the form  \eqref{psdlift} is called an {\em extended formulation} or  {\em PSD-lift} of $P$ and     is extremely useful for optimization purposes. Indeed,  the existence of a PSD-lift immediately implies   that $\min \{\la c, x\ra : x\in P\}=\min\{ \la \pi^\sfT(c), y\ra: y\in  \psd^r \cap \mathcal{L}\}$, and consequently,  linear optimization over $P$  (which can be hard) corresponds to an SDP (which can be solved efficiently). 


%where, $\psd^r$ denotes the cone of PSD matrices, $\mathcal{L}$ denotes an affine subspace,  and $\pi$ a linear projection from the space of $r\times r$ symmetric matrices to $\R^d$.
%while $\pi$ is a linear projection map to $\R^d$.  
 
 To  describe the connection of PSD factorizations with  SDP-lifts, 
let  $S_P$ be the  {\em slack matrix} of $P$,  namely, $S_P$ is a rectangular matrix whose rows are indexed by the facets of $P$, its columns indexed by  extreme points $v_j$,  and the $ij$-entry of $S_P$ corresponds to the slack between the $i$-th facet and the  $j$-th vertex,    $S_{ij}=d_i- c_i^\sfT v_j$.    Generalizing a seminal result by Yannakakis for LPs~\cite{yannakakis}, it was shown independently in \cite{lifts} and \cite{sam} that if $S_P$ admits an $r$-dimensional PSD factorization, the polytope $P$ 
%the PSD-rank of the slack matrix $S_P$ is   
%the smallest $r\in \mathbb{N}$ for which $P$ 
admits a PSD-lift over the cone of $r\times r$  PSD matrices. The proof is also constructive -- given a PSD factorization of $S$, there is an explicit description of $\mathcal{L}$ and $\pi$ that gives rise to $P$.


An important special case of the PSD factorization problem is when the PSD factors are block-diagonal PSD matrices, where both the number of  blocks and the size of each block is fixed,~i.e., 
$A_i,B_j\in (\psd^r)^k.$%\underbrace{\psd^r\times \ldots\times  \psd^r}_{k- times}.$
For a fixed and user-specified $r\in \mathbb{N}$, the least $k\in \mathbb{N}$ for which $X\in \R_+^{m\times n}$   admits a PSD factorization with PSD-factors in $(\psd^r)^k$ is called the $r$-block diagonal PSD-rank  of $X$. In terms of the geometric interpretation of PSD factorizations, block-diagonal PSD factorizations of the slack matrix $S_P$ 
 correspond to  extended formulations of $P$ over  a Cartesian product of  PSD cones, i.e.,  $P=\pi((\psd^r)^k \cap \mathcal{L}).$
In terms of relevance to optimization,  extended formulations over~$(\psd^r)^k$    allow to perform linear optimization over $P$ by solving    block-diagonal SDPs, which can be solved numerically much faster compared to dense SDPs. 
In fact,  most  interior-point algorithms for SDPs are  designed to exploit block-diagonal structure if it present in the problem.  The first systematic study of block-diagonal PSD-lifts was given in \cite{FP13}, where the focus was mainly on lower~bounds. 


%
%Gouveia, Parrilo, and Thomas show that the smallest such $r$ is precisely the PSD-rank of the \emph{slack matrix} $S$, $S_{ij}=d_i- c_i^\sfT v_j$, of the polytope $P$ \cite{lifts,sam}.  The result extends a seminal result by Yannakakis who showed that the smallest LP description of a polytope $P$ is the non-negative rank of $S$  \cite{yannakakis}.  
%
%  To formally describe the connection of PSD factorizations with  SDPs, consider a bounded polytope 
%$$P=\{x\in \R^d: c_i^\sfT x\le d_i, \ i\in [\ell]\}={\rm conv}(v_1,..,v_k),$$ and
%let  $S_P$ be the  {\em slack matrix} of $P$,  i.e., $S_P$ is a rectangular matrix whose rows are indexed by the facets of $P$, its columns indexed by  extreme points $v_j$,  and the $ij$-entry of $S_P$ corresponds to the slack between the $i$-th facet and the  $j$-th vertex, i.e.,    $S_{ij}=d_i- c_i^\sfT v_j$.  

  %Furthermore, it is easy to see that any entrywise nonnegative  matrix  $X\in \R_+^{m\times n}$  admits a PSD factorization, e.g., take  $A_i={\rm diag}(X_{:i})$ and $B_j={\rm diag}(e_j)$, which is a  PSD factorization of size $d$.  
 %For a given polytope $P$, we focus on the  {\em  least size} $r\in \mathbb{N}$ for  which the exists a PSD factorization with $r\times r$ PSD matrices, which is called the {\em positive semidefinite rank}  (psd-rank) of $P$, e.g., see \cite{psdrank} and references therein. 
%  Note that by construction  the slack matrix $S_P$ of a polytope $P$ is entrywise-nonnegative.  Generalizing a seminal result by Yannakakis \cite{yannakakis}, it was shown independently in \cite{lifts} and \cite{sam} that if $S_P$ admits an $r$-dimensional PSD factorization, the polytope $P$ 
%the PSD-rank of the slack matrix $S_P$ is   
%the smallest $r\in \mathbb{N}$ for which $P$ 
%can be expressed as the projection of an affine slice of the cone of $r\times r$  PSD matrices,~i.e., 
%\be\label{psdlift}
%P=\pi(\psd^r \cap \mathcal{L}),
%\ee
%where  $\mathcal{L}$ is an affine subspace of the space of $r\times r$ symmetric matrices and $\pi$ a linear projection from the space of $r\times r$ symmetric matrices to $\R^d$.    An expression of the from  \eqref{psdlift} is called an {\em extended formulation} or  {\em PSD-lift} of $P$ and     is extremely useful for optimization purposes. Indeed,  we  immediately get from  \eqref{psdlift} that linear optimization over $P$ (which can be hard) corresponds to a semidefinite program (which can be solved to arbitrary precision in polynomial time), namely
%$$\min \{\la c, x\ra : x\in P\}=\min\{ \la \pi^\sfT(c), y\ra: y\in  \psd^r \cap \mathcal{L}\}.$$
%The smallest $r\in \mathbb{N}$ for which $P$ has a PSD-lift of size $r$ is just the PSD rank of $S_P$. 


%An NMF of a 
%
% 
%
%
% on this observation, 
%
%Th   generalizing a  
%In 1986–1987 there were attempts [68] to prove P = NP by giving a polynomial-size LP that would solve the traveling salesman problem (TSP). Due to the large size and complicated structure of the proposed LP for the TSP, it was difficult to show directly that the LP was erroneous. In a groundbreaking effort to refute all such attempts, Yannakakis [71] proved that every symmetric LP for the TSP has exponential size (see [72] for the journal version)
%
%The usefulness 
 


\paragraph{Links to quantum information theory.}
Consider two  parties, Alice and Bob,   that try to generate samples $(i,j)$ following some joint distribution $P(i,j)$. For this section, it  is crucial  to   think  of the distribution  $P(i,j)$ as being  arranged in an entrywise  non-negative matrix, and we use $P$ to  simultaneously refer  to both the  distribution and its  matrix  representation.  Clearly, if $P$ is not  a product distribution, Alice and Bob should   either communicate  or share some common information to be able  to generate samples according to $P$. In the {\em correlation generation problem}, the goal is to find  the least amount of shared resources that are needed to achieve this task. The considered resources can be  either  classical (shared randomness), quantum (shared entangled state) or hybrid. 

In the quantum case,   correlation generation  boils down to finding  a quantum state   $\rho \in \psd^{r^2}$ with $\tr(\rho)=1$ and quantum  measurements  $E_i, F_j$ (i.e., $E_i,F_j\in \psd^r$ and $\sum_iE_i=\sum_jF_j=I$) such~that 
 \be\label{quantum}
 P(i,j)=\tr( (E_i\otimes F_j)\rho), \   i\in [m],\ j\in [n].
 \ee 
 The least $r\in \mathbb{N}$ for which a factorization of the form \eqref{quantum} is possible is 
 given by the (logarithm) of  the  psd-rank of the matrix $P$~\cite{qcorr}. Moreover, the proof of \cite{qcorr} is constructive, in the sense that, given a $r$-dimensional  PSD factorization of $P$, there is an  explicit description of a quantum state $\rho \in \psd^{r^2}$ and  measurement operators acting on $\mathbb{C}^r$ that satisfy \eqref{quantum}, e.g., see \cite[Proposition 3.8]{psdrank}. 

% Concretely, consider $P_{i,j}=\tr(A_iB_j)$ with $A_i,B_j\in \psd^r$ and let  $\Sigma_A=\sum_iA_i$ and $\Sigma_B=\sum_jB_j$. Then, the operators $E_i=\Sigma_A^{-1/2}A_i\Sigma_A^{-1/2}$  and $F_j=\Sigma_B^{-1/2}B_j\Sigma_B^{-1/2}$ form  valid quantum measurements and defining the quantum state  $\rho=\psi\psi^\dagger$ where $\psi=(\Sigma^{1/2}_A\otimes \Sigma^{1/2}_B){\rm vec}(I_r)$ it is easy to verify   that
%we have that  $P(i,j)=\tr( (E_i\otimes F_j)\rho)$, %$$
%\begin{aligned}
%& P_{i,j}=\tr(A_iB_j)={\rm vec}(I_r)^\sfT(A_i\otimes B_j){\rm vec}(I_r)\\
%&={\rm vec}(I_r)^\sfT(\Sigma^{1/2}_A\otimes \Sigma^{1/2}_B)(\Sigma_A^{-1/2}A_i\Sigma_A^{-1/2}\otimes \Sigma_B^{-1/2}B_j\Sigma_B^{-1/2})(\Sigma^{1/2}_A\otimes \Sigma^{1/2}_B){\rm vec}(I_r)=\tr(\rho(E_i\otimes F_j)).
%\end{aligned}
%$$

Moving beyond purely quantum protocols, there has been  recent interest   in  hybrid classical-quantum  protocols, motivated by the fact that near-term quantum devices can  only operate reliably on a limited number of qubits  \cite{blockpsd}. Specifically, assuming that their  quantum capabilities are limited to manipulating $s$ qubits,  hybrid classical-quantum protocols that allow    to generate samples  from a joint distribution $P(i,j)$, correspond to PSD factorizations of~$P$ where the PSD factors are block-diagonal, with block-size   at most $2^s$. Moreover, the minimum amount of classical resources required in a classical-quatum protocol with $s$ qubits, is given by the $2^s$-block diagonal PSD-rank  of $P$. 

%The main result in \cite{blockpsd} is to identify a matrix $P$ with PSD-rank 4, whose  $2^s$-block diagonal PSD-rank  is $\log\log n$, i.e., to compensate for a single-qubit shortage in generating $P$, one needs to consume $\log \log n$ classical resources. 


\paragraph{Links to nonnegative matrix factorizations.}
%Consider an entrywise nonnegative   data matrix   $X\in \R_+^{m\times n}$    and a user-specified parameter $r\in~\mathbb{N}$.
 An $r$-dimensional {\em nonnegative matrix  factorization} (NMF) of  $X\in \R_+^{m\times n}$ \cite{PT,Lsnature} is specified by two families  of $r$-dimensional entrywise nonnegative vectors  $a_1,\ldots, a_m\in \R^r_+$ and $b_1,\ldots,b_n\in \R^r_+$  satisfying 
\be\label{nmf}
X_{ij}= \la a_i,b_j\ra,\   i\in [m],\ j\in [n].
\ee
NMF is  a widely used  dimensionality reduction tool that
%
%. Due to the nonnegativity, the factors of lower rank approximation give a natu- ral interpretation: each object is explained by an additive linear combination of intrinsic ‘parts’ of the data
 gives  {\em parts-based representation} of the input data, as   it only allows for additive, not subtractive, combinations.
%NMFs are extremely useful as they give   additive and sparse representations of data.
To make this point clear, note that an equivalent reformulation of an $r$-dimensional  NMF   \eqref{nmf} is   $X=AB$
%\be\label{nmf2}
%X=AB,
%\ee
where $A\in \R^{m\times r}_{+}$ is the matrix whose rows are the $a_i$'s and the matrix $B\in \R_{+}^{r\times n}$ has as columns  the $b_j$'s, or equivalently,
\be\label{nmf2}
X_{:j}\in {\rm cone}(A_{:1}, \ldots, A_{:r}), \ j \in [n].\ee
 The equivalent viewpoint   for NMFs given in \eqref{nmf2} is  more amenable to interpretation, as it  gives a representation of  each column of $X$ (i.e., each data point)  as nonnegative (and thus additive)   combination of the $r$ columns of $A$, and the columns of $B$ give the coefficients of the conic~combination.  %In this setting, the columns of $A$ correspond to a ``sparse basis" that c 
NMF factorizations   have  applications  in many areas,  notable examples including  document clustering \cite{XLG03}, music analysis \cite{fevotte},     speech-source separation  \cite{speech-sep} and  cancer-class identification~\cite{GC05}. For a comprehensive discussion  on  NMFs  the reader is referred to  the survey \cite{gilis} and references~therein.  


NMF factorizations are a special case of PSD factorizations where the $r\times r$ PSD matrices $A_i$ and $B_j$ are {\em diagonal}, i.e.,  we have that  $A_i={\rm diag}(a_i)$ and $ B_j={\rm diag}(b_j)$ for some vectors $a_i,b_j\in\R^r_+$ (recall that a diagonal matrix is PSD iff its diagonal entries are nonnegative). Moreover,  given a PSD factorization of $X$, (i.e., $X_{ij}=\tr(A_iB_j)$) for which all the PSD factors $A_i,B_j$ commute (and thus can be simultaneously diagonalized), corresponds to an NMF factorization.  
In this sense, PSD factorizations  are  a natural non-commutative generalization of  NMF factorizations.
 %corresponds to the problem of finding a nonnegative matrix factorization of $X$. %Indeed, in this case the PSD factorization   $X_{ij}=a_i^\sfT b_j$, can be equivalently written as $X=AB$,  
 %ADD sng about sparsity additivity interpretability.
 
 \paragraph{Interpretability of PSD factorizations.} An equivalent way to define   an {$r$-dimensional} NMF for a data matrix $X$ (cf. \eqref{nmf})  is through the  existence of  a liner mapping $\mathcal{A} : \mathbb{R}^{r} \rightarrow \mathbb{R}^{m}$  satisfying
 \be\label{nmflatent}
 X_{:j}\in \mathcal{A}(\R^r_+) \ \text{ for all }  j\in [n] \quad \text{ and } \quad  \cala(\R^r_+)\subseteq \R^n_+. 
 \ee
% Specifically, $\cala$ is the  linear map $z\mapsto 
%	\mathcal{A}(z) = \left(
%	\langle a_1,z \rangle, \ \ldots \ 
%	,\langle a_m,z \rangle
%	 \right)$, where the $a_i$'s are as in \eqref{nmf}. 
%	 and
Consequently, the mapping $\cala$ (or rather, 
the  image of the extreme rays of the cone $\R^r_+$ under $\mathcal{A}$),  describe a latent space 
that can generate   all data points  $X_{:j}$ via nonnegative combinations. 

Analogously, in the setting of PSD factorizations, the existence of an $r$-dimensional PSD factorization of  $X$ (cf.~\eqref{factorization})  is equivalent to the existence of a linear mapping $\cala: \mathbb{S}^r \to \R^m$ satisfying
 \be\label{psdlatent}
 X_{:j}\in \mathcal{A}(\psd^r) \ \text{ for all }  j\in [n] \quad \text{ and } \quad  \cala(\psd^r)\subseteq \R^n_+. 
 \ee
Comparing  \eqref{nmflatent} and \eqref{psdlatent}, the difference between NMF and PSD factorizations is immediately apparent. In the setting of PSD factorizations the latent pace is {\em infinite-dimensional}, and specifically, it is the  image of the extreme rays of the cone of $r\times r$ PSD matrices (i.e., all matrices $uu^\sfT$ where $u\in \R^r$) under~$\mathcal{A}$. In this  latent space, each data  point $X_{:j}$ is represented by a PSD matrix $B_j\in \psd^r$, and using 
its spectral decomposition  $B_j=\sum_{i=1}^r\lambda_iu_iu_i^\sfT$, leads to the representation
$X_{:j}=\sum_i\lambda_i\cala(u_iu_i^\sfT).$ Additional details and explicit  examples demonstrating the qualitative difference in expressive power  between  NMF and PSD factorizations are given in Section \ref{sec:numerical}. 

\section{Prior Works on PSD Factorizations and Summary of Results}
%\paragraph{High-level  approach.} 
 A canonical  starting point for finding an (approximate) $r$-dimensional PSD factorization of a given  matrix $X\in \R_+^{m\times n}$  is     to solve the non-convex optimization problem
\be\label{bigboss}
\inf  \sum_{i,j}(X_{ij}-\tr(A_iB_j))^2 \quad \text{s.t.}\quad  \ A_1, \ldots, A_m, B_1, \ldots B_n\in \psd^r,
\ee
aiming to  find  an approximate $r$-dimensional PSD factorization that minimizes   the square loss over all entries of $X$. 
Fixing  one of the two families  of matrix variables, say   the $A_i$'s, problem \eqref{bigboss} is  separable with respect to  $B_1,\ldots, B_m$. Consequently,   a reasonable solution approach for \eqref{bigboss}  is to  alternate between updating the $A_i$'s and $B_j$'s by solving the   sub-problems:
\begin{align}
A_i&\leftarrow  \arg \inf~~ \sum_{i,j}(X_{ij}-\tr(A_iB_j))^2 \quad \text{s.t.} \quad  A_1,\ldots, A_m\in \psd^r  \label{alt1}\\
B_j&\leftarrow \arg \inf ~~ \sum_{i,j}(X_{ij}-\tr(A_iB_j))^2 \quad \text{s.t.} \quad   B_1,\ldots,B_n\in \psd^r  \label{alt2}
\end{align}
The two sub-problems   in each update step are symmetric in the variables $A_i$ and $B_j$, with the small modification where we replace $X$ with its transpose.  As such, for the remainder of this discussion, we only focus on the sub-problem \eqref{alt2} corresponding to fixing the $A_i$'s and updating the~$B_j$'s. 
 Moreover, \eqref{alt2} is separable with respect to each variable $B_i$, so it suffices to focus on %the  sub-problem: 
 \be\label{acfsdv}
{\inf}  \sum_{i}(X_{ij}-\tr(A_iB_j))^2 \quad \text{s.t.} \quad  B_j\in \psd^r.
 \ee
%$$\inf \left\{{1\over 2}\sum_i(X_{ij}-\tr(A_iB_j))^2: \  B_j\in \psd^r  \right\}.$$
Lastly, to simplify notation we omit subscripts, and specifically, we denote  by  $x$  the $j$-th column of $X$ and by $B$ the PSD matrix variable~$B_j$.   Defining  $\mathcal{A} : \mathbb{S}^{r} \rightarrow \mathbb{R}^{m}$ to be the linear map 
$	\mathcal{A}(Z) = \left(
	\langle A_1,Z \rangle, \ \ldots \ 
	,\langle A_m,Z \rangle
	 \right),
$  problem~\eqref{acfsdv} can be then equivalently written~as
 \be\label{main}
 %\inf \left\{\|x-\mathcal{A}(B)\|^2: \  B \in \psd^r  \right\}.
 { \inf} ~~ \| x - \mathcal{A} (B) \|_2^2 \quad \mathrm{s.t.} \quad  B \in \psd^r.
 \ee
 
 The optimization problem \eqref{main} is convex, and in fact, falls within  the well-studied class of convex quadratic SDPs. Nevertheless, there is no closed-form solution for this family  of  optimization problems, and consequently,   typical solution strategies  rely on     numerical optimization,  e.g., see~\cite{toh}. 
 

 \paragraph{Summary of results.}    In this paper we introduce  and study an iterative algorithm  (Algorithm~\ref{alg}) we call the {\em Matrix Multiplicative Update} (MMU) algorithm for computing PSD factorizations. The MMU algorithm builds  on the Majorization-Minimization framework, and as discussed in the previous section, the main workhorse is an   iterative algorithm for  the convex quadratic SDP~\eqref{main}.  

From a computational perspective, the iterates of the MMU   algorithm  are updated via  conjugation with appropriately defined matrices,  so our method  has the advantage of being {\em simple to implement} and moreover,  the PSDness of the iterates is {\em automatically guaranteed}. From a theoretical perspective, the squared loss objective is non-increasing along the algorithms' trajectories (Theorem \ref{LSstylethm}) and moreover,  its fixed points satisfy the  first-order optimality  conditions (Theorem~\ref{fixedpointsthm}).  The analysis of the MMU algorithm  relies on the use of several operator trace inequalities (including Von Neumann's trace inequality and Lieb's Concavity Theorem).

An important feature of the MMU  algorithm is that if it is initialized with block-diagonal PSD matrices,  the same block-diagonal structure is {\em preserved throughout  its execution}, which 
    leads to  an algorithm  for calculating block-diagonal PSD factorizations. 
  In particular, in Section \ref{sec:applications} we show that if the MMU  algorithm is initialized with  {\em diagonal PSD matrices}, the iterates remain diagonal PSD throughout,  and as it turns out, our algorithm in this case  reduces to   Lee-Seung's seminal Multiplicative Update algorithm  for   computing NMFs \cite{LS00}. Moreover, we show how to the MMU algorithm can be used as a primitive to calculate PSD factorizations of nonnegative tensors. In terms of numerical experiments,  in Section \ref{sec:numerical} we demonstrate the utility of our method for  both synthetic (random Euclidean Distance matrices) and real data (CBCL image dataset). 
   
 \paragraph{Existing work.} 
    
%ADD: IPO mrethods much bigger size. 
All 
existing algorithms for computing PSD factorizations  employ the alternating minimization approach described in the previous section, where we fix one set of variables and minimize over the other, and essentially boil  down into finding algorithms for  the convex problem~\eqref{main}.

% In the following, we discuss prior works for minimizing \eqref{bigboss} by focusing on the following sub-problem:
%\be\label{small}
%\inf \Big\{\|x-\mathcal{A}(B)\|^2: \  B \in \psd^r  \Big\}.
%\ee

\medskip 
\noindent {\em Projected Gradient Method (PGM).}  The first approach for computing PSD factorizations  is based on  applying PGM to \eqref{main}, alternating  between a gradient step to minimize the objective and  a projection step onto the set of PSD matrices \cite{VGG18}.  The latter projection step uses the following useful fact: Given the spectral decomposition $C=U{\rm diag}(\lam_i)U^\sfT$ of a matrix $C\in \bbS^n$, the projection onto the PSD cone is $U{\rm diag}(\max(0,\lam_i))U^\sfT$ \cite{hig}.  The vanilla PGM has slow convergence rate, so the authors in \cite{VGG18} also propose an accelerated variant that incorporates a momentum term.

\medskip 

\noindent {\em Coordinate Descent.}  The authors in \cite{VGG18} also propose a different algorithm combining the ideas of coordinate descent and  a change of variables that allows them to also control  the rank of the PSD factors, which  was popularized by  the seminal work of Burer and Monteiro for solving rank-constrained SDPs \cite{BM}. 
%explicitly expressing each factor in its PSD factorization to enforce the PSD constraint. 
  Concretely, the authors use the  parameterization  $A_i=a_ia_i^\sfT$, and $B_j=b_jb_j^\sfT$, where $a_i\in \R^{r\times r_{A_i}}$, and $b_j\in \R^{r\times r_{B_j}}$ for some fixed $r_{A_i}, r_{B_j}\in \mathbb{N}$, and optimize using a coordinate descent scheme over  the entries of the matrices $a_i$ and $b_j$.
  %  This approach is frequently associated  with  the seminal work of Burer and Monteiro for solving rank-constrained SDPs \cite{BM}, and has the advantage that the matrices $A_i$ and $B_j$ may be rank deficient. %The BM approach relies on the observation that  an  $n$-by-$n$ psd matrix $X$ with rank $r$ can be written as $X=\sum_{i=1}^rx_ix_i^\sfT=XXT$ for some real vectors $x_1,\ldots, x_r\in \R^{n\times 1}$. 
%Specifically, fixing (in some ad-hoc manner) the ranks $r_{A_i}$ and $r_{B_j}$ for each $A_i$ and $B_j$ respectively, it follows that there exists matrices $a_i\in \R^{r\times r_{A_i}}$ and  $b_j\in \R^{r\times r_{B_j}}$ such that  $A_i=a_ia_i^\sfT$ and $B_j=b_j{b_j}^\sfT$.  
In this setting,    problem \eqref{main}  
%\be\label{BM}
%{ \inf} ~~ \| x - \mathcal{A} (bb^\sfT) \|_2^2 \quad \mathrm{s.t.} \quad  b\in \R^{r\times r_B},
% \ee
 is a quartic polynomial in the entries of $b$.  Thus, its gradient is a cubic polynomial, 
%as the following problem over the $a_i$'s and $b_j$'s:
%\be\label{factorformulation}
%{\inf} \Big\{ \sum_{i,j}(X_{ij}-a_i^\sfT b_j)^2: \ a_i\in \R^{r\times r_{A_i}},  b_j\in \R^{r\times r_{B_j}}\Big\}.
%\ee 
%The algorithm proceeds by fixing one set of variables -- say the $a_i$'s -- while updating the other set -- say the $b_j$'s.  The resulting problem entails the minimization of a degree four polynomial over $\R_+$, 
and its roots can be found  using  Cardano's method (and careful book-keeping). %an explicit formula for  the roots of a cubic polynomial (as Cardano's method).
 
% We conclude with a note on the convergence properties of the coordinate descent method: Every limit point of the sequence of iterates generated by the CD method is a stationary  point if the minimum in each CD subproblem is uniquely attained (assuming a convex objective function and convex constraint sets) \cite{Ber}.  Nevertheless, note that these assumptions are not necessarily satisfied in this case.   Lastly, we note that  an additional desirable  feature of the factor-based formulation~(\eqref{factorformulation}) is that   it allows to explicitly  control the rank  of the PSD factors, i.e., the $r_j$'s. 


\medskip 
\noindent {\em Connections to Affine Rank Minimization and Phase Retrieval.}  A different set of algorithms developed in \cite{LF20, LF20b, LLTF20} is based on the connections between computing PSD factorizations with the affine rank minimization (ARM) and the phase retrieval (PR) in signal procesing.  
First, recall that the PSD-ARM problem focuses on  recovering a low-rank matrix from affine measurements:
$$
 \min ~~ \rank(B) \quad \text{s.t.} \quad   \ \cala(B)=x, \ B\in \psd^r.
$$
Here, $\cala$ is a known linear map representing measurements while $x$ is known vector of observations. Due to the non-convexity of the rank function, a useful heuristic initially popularized in the control community  is to replace the rank by  the trace function, e.g., see \cite{MP} and \cite{fazel}, in which case the resulting problem is an instance of an SDP.  A different  heuristic for   PSD-ARM is to find a PSD matrix of rank at most $k$ that  minimizes the squared loss function, i.e., \be\label{cdsfvsdfv}
 \inf~~ \|x-\cala(B)\|_2^2 \quad \text{s.t.} \quad  B\in \psd^r, \ \rank(B)\le k,
\ee
where alternatively, the rank constraint can be enforced  by parametrizing the PSD matrix variable $B\in \psd^r$ as $B=bb^\sfT$ with $b\in \R^{r\times k}$. 
The point of departure for the works  \cite{LF20, LLTF20, LF20b} is that problem~\eqref{cdsfvsdfv}  corresponds exactly to  the sub-problem \eqref{main} encountered in any alternate minimization strategy for computing  PSD factorizations,   albeit with an additional  rank constraint. In view of this, any  algorithm  from the signal processing literature developed for ARM can be applied to \eqref{main}.


%can be optimized using existing methods in the literature that were developed for phase retrieval and ARM.

The main algorithms considered in \cite{LF20, LF20b, LLTF20}  are Singular Value Projection (SVP)  \cite{SVP},   Procrustes Flow \cite{procrsustes}, and variants thereof.
%which  involves an initialization phase   based on SVP  followed by a  second phase which  essentially performs gradient descent with a meticulously  chosen step size. 
In terms of convergence guarantees,  for affine maps $\mathcal{A}$  obeying the  Restricted Isometry Property \cite{RIP}, both algorithms converge to an optimal solution. Nevertheless, it is unclear whether these guarantees carry over when applied to the PSD factorization problem. 
  % LS's algorithm is perhaps the most widely used  method for computing  NMFs, its pervasiveness  owing  to its good practical performance   and its  simplicity  of implementation.
 
% This  leads to the first algorithm  for calculating block-diagonal PSD factorizations. Additionally, 
 %using an alternate optimization approach, our algorithm can be also used to calculate PSD-factorizations for tensors. 
\paragraph{Roadmap.} In Section \ref{sec2} we derive our MMU algorithm for computing PSD factorizations and in Section \ref{sec:fp} we show that its fixed points   correspond to KKT points. In Section \ref{sec:applications} we give various theoretical applications of the MMU algorithm and in Section \ref{sec:numerical} we go from theory to practise and apply the MMU algorithm to synthetic and real datasets.   


%From a theoretical and computational standpoint,  our algorithm   enjoys  four important properties: $(i)$  it is simple to implement as it acts by  $(ii)$  the update rule preserves positive
%PSDness of the updates is automatically satisfied as the new iterates are obtained from the old iterates   by congruence scaling with the matrix geometric mean of appropriate PSD matrices,
 %$(iii)$  t Our main technical result is  Theorem \ref{thm:domination_general}, and its analysis 


%
% Interestingly, our algorithm can be also viewed as  a  non-commutative extension of Lee-Seung's~(LS) seminal multiplicative update algorithm  for   computing NMFs \cite{LS00}. LS's algorithm is perhaps the most widely used  method for computing  NMFs, its pervasiveness  owing  to its good practical performance   and its  simplicity  of implementation. 
 
% Specializing our algorithm to diagonal PSD matrices, we recover LS's algorithm, but more importantly, our approach allows to give a  natural interpretation of the  derivation of LS's algorithm,  by making the search of mulitplicative updates explicit. 
% 




% which (1) retains the simplicity of implementation that the multiplicative update algorithm for NMF enjoys (2) ensures that updates remain PSD by congruence scaling with the matrix geometric mean of appropriate PSD matrices, and (3) the squared loss objective is non-increasing along the trajectories of the algorithm and fixed points correspond to critical points.   
 
   
   

%    LS's algorithm is a widely used  method for computing an $r$-dimensional NMF of a matrix, and also relies on the idea of finding an NMF that (approximately) minimizes  the square loss (or KL divergence) over all entries, using alternate minimization. Drawing a parallel to   the PSD case, the sub-problem analogous to \eqref{main}  that Lee-Seung are faced with at each iteration  is:
% \be\label{NLS}
%    \underset{b}{ \inf} ~~ \| \bx_j - \mathcal{A} (b) \|_2^2 \quad \mathrm{s.t.} \quad  b \in \mathbb{R}_+^r,
%\ee
%    where in the LS setting, 
%      $\mathcal{A} : \mathbb{S}^{r} \rightarrow \mathbb{R}^{m}$ is the linear map $z\mapsto 
%	\mathcal{A}(z) = \left(
%	\langle a_1,z \rangle, \ \ldots \ 
%	,\langle a_m,z \rangle
%	 \right),$
%and $a_1,\ldots, a_m$ are fixed entry-wise non-negative vectors.   
%
%Note that \eqref{NLS} is  a  non-negative least squares problem, and although convex, there is no closed-form solution and   most existing  solution strategies   rely on  numerical optimization. On the other hand, building on the Majorization-Minimization framework (see Section \ref{sec2}), Lee and Seung introduced   an iterative method (see  \eqref{LSalg}) which is (1)   simple to implement (2)  non-negativity of the updates is automatically preserved by scaling with positive diagonal matrices (3)  the squared loss (and KL) objective is non-increasing along the trajectories of the algorithm and fixed points correspond to critical points.  


   
      

==> manuscript PSD case: arxiv/sec_kkt_CURRENT.tex <==
\section{Fixed Points of the MMU Algorithm}\label{sec:fp}

In this section, we show that the fixed points of the MMU algorithm satisfy the Karush-Kuhn-Tucker~(KKT)   optimality conditions for problem \eqref{bigboss}. % To this end, we begin by describing the KKT conditions for our problem.
 Letting $\{A_i^*\}_{i\in [m]},\{M^*_i\}_{i\in [m]}$ and $ \{B^*_j\}_{j\in [n]}, \{\Lambda^*_j\}_{j\in [n]}$ be   pairs of primal-dual optimal solutions of \eqref{bigboss} with zero duality gap, it is straightforward to verify that the KKT conditions  are 
$$
\begin{aligned}
& \tr(A^*_iM^*_i)=\tr(B^*_j\Lambda^*_j)=0, \quad  i\in [m], j\in [n] \\
&\mcb^\sfT (X_{: i})-[\mcb^\sfT\mcb] (A^*_i)=M^*_i, \quad i\in [m]\\
& \cala^\sfT (X_{: j}) -[\cala^\sfT \cala] (B^*_j)=\Lambda^*_j, \quad j \in [n].
\end{aligned}
$$
%
% Due to the symmetry in the variables $\{A_i\}$ and $\{B_j\}$ in \eqref{bigboss}, we focus on the setting where the $A_i$'s are fixed and the $B_j$'s are the only variables in the problem.  To simplify notation, we describe the sub-problem for a fixed index $j$, and we omit the dependency on $j$.  The objective, augmented with the Lagrangrian to incorporate the PSD constraint, is given as follows:
%\begin{equation*}
%\| \mathcal{A}(B) - x \|^2 + \mathrm{tr}(BW).
%\end{equation*}
%Here, $W \in \mathbb{S}^n_+$ is the dual variable associated with the PSD constraint.  At first order optimality, the primal optimal variable $B^*$ and the dual optimal variable $W^*$ satisfy the following first order optimality condition:
%\begin{equation} \label{eq:kkt_foc}
%(\mathcal{A}(B^*) - x )^\sfT \mathcal{A} + W^* = \sum_k (\mathrm{tr}(A_k B^*) - x_k) A_k + W^* =  0,
%\end{equation}
%and the following complementary slackness condition:
%\begin{equation*}
%\mathrm{tr}(B^* W^*) = 0.
%\end{equation*}
Furthermore, assuming that the primal optimal solutions $\{A^*_i\}_{i\in [m]}$ and  $\{B^*_j\}_{j\in [n]}$ are all  {\em positive definite}, it follows immediately from the complementary slackness conditions that $M^*_i=\Lambda^*_j=0$ for all $i\in [m], j\in [n]$. Consequently, in the special case of positive definite optimal solutions $\{A^*_i\}_{i\in [m]}$ and  $\{B^*_j\}_{j\in [n]}$ , the KKT conditions reduce to
\be\label{KKT}
\mcb^\sfT (X_{: i})=[\mcb^\sfT\mcb] (A^*_i), \ i\in [m] \quad \text{ and } \quad
 \cala^\sfT (X_{: j}) =[\cala^\sfT \cala] (B^*_j), \ j \in [n].
\ee
%We now show that positive  definite fixed points of our update rule \eqref{updaterule}  satisfy the KKT conditions~\eqref{KKT}.
%the   it is further known that the primal optimal variable $B^*$ is \emph{positive definite}.  Then the dual optimal variable $W^*$ must be zero, and in which case \eqref{eq:kkt_foc} reduces to:
%\begin{equation*}
%( \mathcal{A}(B^*) - x )^\sfT B^*= 0.
%\end{equation*}

%Let $\{ A_1^*,\ldots, A_m^* \}$ and $\{B_1^*,\ldots,B_n^*\}$ be first order stationary points of the optimization instance in \eqref{bigboss}, and let $\{ Z_1^*,\ldots, Z_m^* \}$ and $\{W_1^*,\ldots,W_n^*\}$ be positive semidefinite matrices representing the dual variables associated to the constraints $A_i \succeq 0$ and $B_j \succeq 0$ respectively.  In addition to the first order optimality conditions, the primal variables $\{A_i^*\}$, $\{B_j^*\}$ and the dual variables $\{Z_i^*\}$, $\{W_j^*\}$ also satisfy the following complementary slackness conditions:
%\begin{equation*}
%\begin{aligned}
%\mathrm{tr}(Z^*_i A^*_i ) = \mathrm{tr}(W^*_i B^*_j) &=0\\
%-\sum_{j}(X_{ij}-\tr(A^*_iB^*_j))B^*_j(k,l)-Z^*_i(k,l)&=0\\
%-\sum_{i}(X_{ij}-\tr(A^*_iB^*_j))A^*_i(k,l)-W^*_j(k,l)& =0.
%\end{aligned}
%\end{equation*}
%Suppose it is further known that the matrices $A^*_1, \ldots, A^*_m$, $B^*_1, \ldots, B^*_n$ are \emph{positive definite}.  By complementary slackness, we have $Z^*_i=W^*_j=0$, in which case the above system of equations reduces to the following:
%\be\label{KKTcompact}
%\mcb^\sfT (X_{: i})=[\mcb^\sfT\mcb] (A^*_i)\ \text{ and } 
%\cala^\sfT (X_{: j}) =[\cala^\sfT \cala] (B^*_j).
%\ee

%\begin{proposition} \label{thm:kkt_prelimpropn}
%Let $B$ and $Y$ be positive definite matrices.  Suppose it is known that $B = R Y R$, where $R = Z \# B$ with $Z$ positive definite.  Then $Y=Z^{-1}$.
%\end{proposition}
%
%\begin{proof}
%Since $B$ and $Y$ are positive definite, $R = Z \# B$ is also positive definite.  We then have $R^{-1} = Z^{-1} \# B^{-1}$.  Subsequently, $Y = R^{-1} B R^{-1} = (Z^{-1} \# B^{-1}) B (Z^{-1} \# B^{-1}) = Z^{-1}$.
%\end{proof}
Based on the preceding discussion, in the next result (whose proof follows by Lemma \ref{thm:kkt_actualresult} in the  Appendix) shows that we can interpret our MMU algorithm as a fixed-point method for satisfying the KKT optimality conditions corresponding to  problem \eqref{bigboss}.
\begin{theorem}\label{fixedpointsthm}
If $\{A_i\}_{ i\in [m]}$  and $\{B_j\}_{j\in [n]}$  are positive definite fixed points of the update rule of the MWU algorithm given  in~\eqref{updaterule}, then they also satisfy the KKT conditions \eqref{KKT}.
\end{theorem}

%The proof of this result is also deferred to . 
%Furthermore, as the $A_i$'s are positive  definite,  we have that $\mathcal{A}^{\sfT} x=\sum_i x_iA_i$ is also positive definite.  The result follows by taking $Y = \mathcal{A}^{\sfT} x$ and $Z = ([\mathcal{A}^{\sfT} \mathcal{A}] (B))^{-1}$ in Proposition \ref{thm:kkt_prelimpropn}.
%Consequently, the geometric mean $R = ([\mathcal{A}^{\sfT} \mathcal{A}] (B))^{-1}\#B$ is positive definite, and $R^{-1} B R^{-1}=\mathcal{A}^\top x$.  On the other hand, consider the matrix equation $Z B Z = \mathcal{A}^\top x$ in the variable $Z$.  Following the properties of the geometric mean, the matrix $B^{-1} \#  (\mathcal{A}^\top x) $ is the unique positive definite solution.  It then follows that $R^{-1} = B^{-1} \#  (\mathcal{A}^\top x)$, and hence $R = B \# (\mathcal{A}^\top x)^{-1}$.
%It follows 
%\be\label{vsbvdsfb}
%(B^{-1}\#[\mathcal{A}^{\sfT} \mathcal{A}](B)) B(B^{-1}\#[\mathcal{A}^{\sfT} \mathcal{A}](B))=[\mathcal{A}^{\sfT} \mathcal{A}](B).
%\ee
%Using the inversion property $(X\#Y)^{-1}=X^{-1}\#Y^{-1}$ and the commutativity property $X\#Y=Y\#X$ of the geometric mean, it follows that the left-hand side of \eqref{csvs} is equal to the left-hand side of Equation \eqref{vsbvdsfb}. Combining the two equations, it  follows that $ \mathcal{A}^\top x=[\mathcal{A}^{\sfT} \mathcal{A}](B)$, and the proof is concluded. 

%It is easy to verify that the fixed points of our update scheme satisfy the KKT conditions.  Conversely, if the set of variables $\{A_i^*\}$ and $\{B_j^*\}$ satisfy the KKT conditions and are each positive definite, then Corollary \ref{thm:kkt_actualresult} tells us that they are fixed points of our update step.

\if0
\vspace{20mm}

In this section we show that fixed points of the update rule $$B^{\mathrm{new}} = T^{-1}(\mathcal{A}^\sfT(x))=Q^{-1}\mathcal{A}^\sfT(x)Q^{-1},$$
where 
$$Q=\bo^{-1}\#[\mathcal{A}^{\sfT} \mathcal{A}] (B_{\mathrm{old}}),$$ correspond to first-order stationary points of  the optimization problem:
\be\label{cvsvsd}
\inf \left\{{1\over 2}\sum_{i,j}(X_{ij}-\tr(A_iB_j))^2: \ A_j, B_j\in \psd^r  \right\}.
\ee
%Note that 
%$${ \partial f\over \partial A_i(k,l)}=-\sum_{j}(X_{ij}-\tr(A_iB_j))B_j(k,l)$$ 
%and 
%$${ \partial f\over \partial B_j(k,l)}=-\sum_{i}(X_{ij}-\tr(A_iB_j))A_i(k,l)$$ 
%The Lagrangian is
%$$\mathcal{L}(A_i,B_j, Z_i,W_j)={1\over 2}\sum_{i,j}(X_{ij}-\tr(A_iB_j))^2-\sum_{i=1}^m\la Z_i, A_i\ra -\sum_{j=1}^n\la W_i,B_j\ra$$ 
%and the dual function becomes 
%$$g(Z_i,W_j)=\inf_{A_i,B_j}\mathcal{L}(A_i,B_j, Z_i,W_j)$$
%Let $A^*_i,B^*_j,$ and  $Z^*_i,W^*_j$  a pair o primal/dual optimal solutions. 
Besides  primal and dual feasibility, the KKT conditions corresponding to \eqref{cvsvsd}  are given by: 
$$
\begin{aligned}
\la  Z^*_i, A^*_i\ra =\la W^*_i,B^*_j\ra &=0\\
-\sum_{j}(X_{ij}-\tr(A^*_iB^*_j))B^*_j(k,l)-Z^*_i(k,l)&=0\\
-\sum_{i}(X_{ij}-\tr(A^*_iB^*_j))A^*_i(k,l)-W^*_j(k,l)& =0.
\end{aligned}
$$
Consequently, for  a positive definite optimal solution $A^*_1, \ldots, A^*_m$, $B^*_1, \ldots, B^*_n$ of \eqref{cvsvsd},    we have that $Z^*_i=W^*_j=0$ and thus, the  KKT conditions reduce to:
$$
\begin{aligned}
\sum_{j=1}^m(X_{ij}-\tr(A^*_iB^*_j))B^*_j(k,l)&=0\\
\sum_{i=1}^n(X_{ij}-\tr(A^*_iB^*_j))A^*_i(k,l)& =0.
\end{aligned}
$$
Equivalently, defining   the linear mappings: $$
  \mcb^\sfT (y)=\sum_{i=1}^my_iB^*_i \  \text{ and } \cala^\sfT(x)=\sum_{j =1}^n x_iA^*_i,
 $$
the KKT conditions can be written succinctly as:
 
\be\label{KKTcompact}
\mcb^\sfT (X_{: i})=[\mcb^\sfT\mcb] (A^*_i)\ \text{ and } 
\cala^\sfT (X_{: j}) =[\cala^\sfT \cala] (B^*_j).
\ee
\begin{theorem}Let $A_1,\ldots, A_n, B_1,\ldots, B_m$  be positive definite matrices that are fixed points of the update rule for PSD factorization, i.e., 
 \be
 \bal 
        A^i&=([\mcb^{\sfT} \mcb] (A^i)^{-1}\#A^i)\mcb^\top(X_{ i : }) ([\mcb^\sfT \mcb] (A^i)^{-1}\#A^i)\quad  i\in [n]\\
  B^j&=([\mathcal{A}^{\sfT} \mathcal{A}] (B^j)^{-1}\#B^j)\mathcal{A}^\top(X_{: j}) ([\mathcal{A}^{\sfT} \mathcal{A}] (B^j)^{-1}\#B^j)\quad   j\in [m].
      \eal 
      \ee
Then, we have that
\be
\mcb^\sfT (X_{: i})=[\mcb^\sfT\mcb] (A^i)\ \text{ and } 
\cala^\sfT (X_{: j}) =[\cala^\sfT \cala] (B^j).
\ee
 
\end{theorem}


\begin{proof}By symmetry it suffices to only consider the $B_j$'s. As $B_j$ is a fixed point we have 
 $$ B^j=([\mathcal{A}^{\sfT} \mathcal{A}] (B^j)^{-1}\#B^j)\mathcal{A}^\top(X_{: j}) ([\mathcal{A}^{\sfT} \mathcal{A}] (B^j)^{-1}\#B^j).
$$
Moreover, since $B_j$ is positive definite (by assumption), it also follows that  $[\mathcal{A}^{\sfT} \mathcal{A}] (B_j)$ is positive definite. Consequently, their geometric mean  $([\mathcal{A}^{\sfT} \mathcal{A}] (B^j)^{-1}\#B^j)$ is positive definite, and we get
 \be\label{csvs}
 ([\mathcal{A}^{\sfT} \mathcal{A}] (B^j)^{-1}\#B^j)^{-1} B^j([\mathcal{A}^{\sfT} \mathcal{A}] (B^j)^{-1}\#B^j)^{-1}=\mathcal{A}^\top(X_{: j}).
\ee
On the other hand, by definition, the geometric mean $C\#D$ is the unique positive solution of  
$XC^{-1}X=D,$ i.e., we have that $(C\#D)C^{-1}(C\# D)=D.$ In particular, we get that
\be\label{vsbvdsfb}
(B_j^{-1}\#[\mathcal{A}^{\sfT} \mathcal{A}](B_j)) B_j(B_j^{-1}\#[\mathcal{A}^{\sfT} \mathcal{A}](B_j))=[\mathcal{A}^{\sfT} \mathcal{A}](B_j).
\ee
Using the inversion property $(X\#Y)^{-1}=X^{-1}\#Y^{-1}$ and the commutativity property $X\#Y=Y\#X$ of the geometric mean, it follows that the left-hand side of Equation \eqref{csvs} is equal to the left-hand side of Equation \eqref{vsbvdsfb}. Combining the two equations, it  follows that $ \mathcal{A}^\top(X_{: j})=[\mathcal{A}^{\sfT} \mathcal{A}](B_j),
$ and the proof is concluded. 
\end{proof}





  
   %\begin{lemma}[
%
%label{thm:bhatia_9_8_16}
%	
%\end{lemma}

%\begin{proof}[Proof of Lemma \eqref{thm:bhatia_extended}]
%	Apply Lemma \eqref{thm:bhatia_9_8_16} with $k=2$ repeatedly.
%\end{proof}





%Here, $\Lambda$ is a linear invertible operator $\mathbb{S}^{n} \rightarrow \mathbb{S}^{n}$.  
%
%One appropriate generalization of diagonal scaling is the operator corresponding to conjugation by invertible matrices.  One perspective why this is the correct generalization is because a diagonal matrix preserves the sparsity of the input vector, while conjugation by an invertible matrix preserves the rank of the input matrix.  From a computational perspective, performing conjugation with invertible matrices is considerably cheaper than applying a generic operator $\Lambda$, which has dimensions $O(q^2) \times O(q^2)$.
%
%As such, our immediate goal is to seek a linear invertible operator corresponding to conjugation by invertible matrices such that
%\begin{equation*} \label{eq:psd_settozero}
%	B_{\mathrm{old}} - \Lambda^{-1} \left( [\mathcal{A}^{\sfT} \mathcal{A}] (B_{\mathrm{old}}) \right) = 0.
%\end{equation*}
%
%
%
%A important basic fact about the geometric mean is that its definition is symmetric in its arguments.
%\begin{proposition}
%	Suppose $X,Y$ are positive definite matrices.  Then $M_0(X,Y) = M_0(Y,X)$.
%\end{proposition}
%
%We define the operator $\Lambda$ as
%\begin{equation*}
%	\Lambda (Z) = W Z W
%\end{equation*}
%where
%\begin{equation*}
%	W = M_0( [\mathcal{A}^{\sfT} \mathcal{A}] (B_{\mathrm{old}}),B^{-1}_{\mathrm{old}}) .
%\end{equation*}
%It is easy to check that our proposed choice of $\Lambda$ satisfies \eqref{eq:nmf_settozero}.  
%
%It follows that our update rule is
%\begin{equation*}
%	B_{\mathrm{new}} = \Lambda^{-1} ( \mathcal{A}^{\sfT} \bx ).
%\end{equation*}
%Note that because the matrix $\mathcal{A}^{\sfT} \bx$ is positive defininte, the resulting update is also positive definite.
%
%
%Equivalently, we solve 
%$$\inf \left\{\sum_j{1\over 2}\|X_{\cdot j}-AB_{\cdot j}\|^2: A,B \ge 0\right\}.$$
%Fix a matrix $A$ of full column rank.  Thus, it suffices to solve:
%$$\inf \left\{{1\over 2}\|X_{\cdot j}-AB_{\cdot j}\|^2:  B_{\cdot j}\ge 0\right\}.$$
%Dropping subscripts for notatinal convenience, we need to solve
%$$\inf \left\{{1\over 2}\|x-Ab\|^2: b\in \R_+^{p}\right\}, $$
%where $x,A$ are fixed. 
%Define 
%$$f(b)={1\over 2}\|x-Ab\|^2.$$
%The Hessian $H_f(b)$ is given by $A^{\sfT}A$,
%%As the matrix $A$ is entrywise nonnegative, we may use Theorem \eqref{thm:uppboundnonnegative} with  $B=H_f(b)=A^{\sfT}A$, 
%which is PSD and also entrywise nonnegative. Thus, we can use either Theorem \eqref{thm:1} or Theorem \eqref{thm:2}. Note that, Theorem  \eqref{thm:1} is uninteresting as in this case, the updates are given by  
%$$b^{new}=b^{old}-(A^{\sfT}A)^{-1}(A^{\sfT}Ab^{old}-A^{\sfT}x)=(A^{\sfT}A)^{-1}A^{\sfT}x, $$
%i.e., they are constant. 
%
% 
% 



%In the po matrix factorization (PSF) problem  the goal  is to identify   two entrywise non-negative matrices $W\in \R_+^{n\times r}$ and $ H\in \R_+^{r\times m}$  $) such that the matrix product $WH$ approximates $V$,  where the precise sense of approximation    depends  on  the application of interest.

%
%There are several  practically efficient algorithms for calculating (approximate) NMFs. The starting point for the majority of existing  approaches is the non-convex~program% in the matrix variables $W,H$
%\begin{equation}\label{main}\tag{NMF}
%\min_{W\in \R_+^{n\times r}, H\in \R_+^{r\times m}} F(W,H):=\| V-WH\|_F^2,
%\end{equation}
%
% Going beyond the BCD framework,  the multiplicative update (MU) rule introduced in~\cite{LS01}
%  is by far the most popular algorithm for NMF. In the MU framework, the updates are given by
%$$W_{t+1}=  W_t\circ {VH_t^\sfT \over W_tH_tH_t^\sfT} \quad H_{t+1}= H_t\circ {W_{t+1}^\sfT V\over W_{t+1}^\sfT W_{t+1}H_t},$$
%where $X/Y$ denotes  the componentwise  division of two matrices. \cite{LS01}  showed using a majorization-minimization  approach, e.g., see \cite{SBP},
%%\sum_{k,\ell}(A_{k,\ell}-\sum_\mu W_{k,\mu}H_{\mu,\ell})^2$$
%%We now calculate the derivative of this with respect to $H_{ij}$. Note that the only terms in the sum that contain $H_{ij}$ (anf thus have nontrivial derivative) are
%%Taking the derivative of this wrt $H_{ij}$ we get
%%$$-2\sum_k (A_{kj}-W_{ki}H_{ij})W_{ki}.$$
%%Now, note that
%%$$\sum_k A_{kj}W_{ki}=\sum_kW^\sfT_{ik}A_{kj}=(W^\sfTA)_{ij}$$
%%and
%%$$\sum_k W_{ki}H_{ij}W_{ki}=\sum_kW^\sfT{ik}W_{ki{H_{ij}.$$
% that under the MU  rule, the objective
%function $\| V-WH\|_F^2$ is non-increasing. However, it has  long been observed  that the MU rule  may fail  to converge to  a first-order stationary point, e.g. see  \cite{GZ05}.
%Indeed, only when  the MU method converges to a fixed point  $(W,H)$  with strictly positive entries
%%we have  that $\nabla_W F=\nabla_HF=0$, implying that $(W,H)$
%this is also  a KKT point.  An important limitation of  the MU update rule is that it cannot be implemented concurrently (as $H_{t+1}$ depends on $W_{t+1}$).  \cite{Lin07} further elaborates on  the  difficulties in proving convergence of the  MU algorithm, while establishing convergence  of a close variant of Lee-Seung's~method.
%


%\subsection{The majorization-minimization paradigm}


%
%\subsection{Nonnegative factorizations}
% For a matrix $Y$ let $Y_{ i\cdot}$ be its $i$-th row and $Y_{\cdot j}$ its $j$-th column. 
%
%Consider an entrywise nonnegative $n\times m$ matrix $X\in \R^{n\times m}_+$. A {\em nonnegative matrix factorization} (NMF) of $X$ is given by 
%\be\label{NMF}
%X=AB, \text{ where } A\in \R^{n\times k}_+, \ B\in \R^{k\times m}_+.
%\ee
% NMF factorizations always exist (e.g. take $A=X, B=I_m$ or $A=I_n, B=X$). 
% 
% The least  $k$ for which an NMF exists is called the {\em nonnegative rank of $X$}, denoted by $rank_+(X)$. Note that $rank_+(X)\le \min \{m,n\}$. 
%Finding the nonnegative rank is hard \cite{vavasis}. 
%
%To put NMFs into context, if we drop the requirement that $A,B$ are entrywise nonnegative, then this just corresponds to the usual rank of the matrix~$X$.  
%
%\medskip 
%
%There's two ways to understand \eqref{NMF}. First, it can be equivaletly re-written~as: 
%\be\label{NMFgram}
%X_{ij}=\la A_{i\cdot},B_{\cdot j}\ra, \ \forall i=1,..,n,\ j=1,..,m,
%\ee
%where 
%%$a_i$ is the $i$-th row of $A$, $b_j$ the $j$-th column of $B$, and 
%$\la \cdot, \cdot \ra$ 
%the standard inner product of vectors. In other words, in a NMF we are looking for entrywise nonnegative vectors $a_1,..,a_n,b_1,..,b_m\in \R^k_+$ (for some $k\ge 1$) such that, the $ij$ entry of $X$ is given by the inner product of $a_i$ and $b_j$. 
%
%Second,  \eqref{NMF}  can be equivalently rewritten as: 
%\be\label{NMFatomic}
%X_{\cdot j} =\sum_{i=1}^kA_{\cdot k} B_{\cdot j}(i),
%\ee
%where $B_{\cdot j}(i)$, is the $i$-th entry of the $j$-th column of $B$. 
%
%\subsection{Motivation I}
%Formulation \eqref{NMFatomic} provides strong motivation  for studying NMFs. As an example, in text-mining applications  the matrix  $X$ is  a word-document incidence matrix. Concretely,  fix $n$ words in the english language and consider $m$ documents $d_1,..,d_m$ in English. Then,  the $j$-th column of $X$ is defined as follows
%$$
%X_{. j}(i)=
%\begin{cases}
%1, \text{ if } i\in d_j\\0, \text{ otherwise}.
%\end{cases} 
%$$
% Given such a matrix  $X$, a NMF as described  in \eqref{NMFatomic}, identifies ``$k$ topics" (i.e., the $k$ columns of $A$) such that, every document (i.e., every column of $X$) can be expressed  as a nonnegative combination of the $k$-topics. %Note that as we are working with linear combinations with {\em nonnegative  entries}, the model is additive. 
%
%There's other natural choices for $X$, e.g., instead of just incidence we can put the number of times word $i$ appears in document $j$, see \cite{gilis}.  
%
%As far as I know, the interpretation of NMFs given in \eqref{NMFgram} is not as useful.  Nevertheless, I vaguely recall that  Cedric mentioned something along these lines but I forget the details.~Vincent?
%
%\subsection{Motivation II, Linear lifts}
%
%Consider the unit ball of the  $\ell_1$ norm, i.e., 
%$$B=\{ x\in \R^n: \sum_{i=1}^n |x_i| \le 1\}.$$
%This can be re-written as 
%$$B=\{ x\in\R^n: \sum_{i=1}^n \pm x_i\le 1\}$$ 
%which is a {\em linear description} that involves {\em an exponential number of inequalities}. 
%This description is not useful if we want to optimize over this set. 
%Nevertheless, there's a clever work-around. For this, note that
%$$B=\{x\in \R^n: \ \exists y\in \R_+^n \text{ such that  } |x_i|\le y_i, \sum_{i=1}^n y_i=1\}$$
%To see the non-trivial direction, if $\sum_{i=1}^n |x_i|\le 1$ set $y_i=|x_i|+(1-\sum|x_i|)/n$. 
%
% This second description,  is defined by  $3n$ linear inequalities and $2n$ variables. The moral here is that by introducing $n$ additional variables, we can define $B$ using $3n$ linear constraints, as opposed to $2^n$ constraints, which we used  in our first naive attempt. 
%%This leads to the notion of {\em extended formulations}. 
%This leads to the following definition:
%
%\begin{definition}A polytope $P=\{x\in \R^n: Ax\le b\}$ has an $\mathbb{R}^k_+$  lift if there exists a polytope 
%$$Q=\{(x,y): Ax+By=\gamma, \ y\in \R^k_+\}$$ 
%such that 
%$$\pi_x(Q)=P,$$
%where $\pi_x$ is juts the coordinate projection onto the $x$-coordinates.
%\end{definition}
%
%The connection with NMF factorizations is given in the following beautiful theorem. 
%
%
%\begin{theorem}[Yannakakis] Consider a polytope 
%$$P=\{x: Ax\le b\}={\rm conv}(v_1,..,v_m).$$ Let $S_P$ be the  {\em slack matrix} of $P$, i.e., the matrix whose rows are indexed by the facets of $P$, its columns by its vertices,  and  $S_{ij}=b_i-\la A_{i\cdot},v_j\ra$.   Then,
%\begin{itemize}
%\item If the slack matrix of $P$ has nonnegative rank $\le k$ then $P$ has a $\mathbb{R}^k_+$-lift.
%\item If $P$ has an $\mathbb{R}^k_+$ lift then  its slack matrices have nonnegative rank $\le k$.
%\end{itemize}
%%Notice that the freedom to choose a slack matrix comes from the fact that the description of $P$ given by $A$ does not have to be a minimal description, i.e., a facet description. 
%\end{theorem}
%
%\subsection{Positive semidefinite (PSD) factorizations}
%
%{\bf Background:} A real symmetric matrix is positive semidefinite (PSD) if all its eigenvalues are nonnegative. We denote by $\psd^n$ the set of $n\times n$ PSD matrices. We consider  the space of  symmetric $n\times n$ matrices as an inner product space where $\la A,B\ra:={\rm trace}(AB).$
%
%\medskip 
%
%Consider an entrywise nonnegative $n\times m$ matrix $X\in \R^{n\times m}_+$. A {\em PSD  factorization}  of $X$ is given by 
%\be\label{PSD}
%X_{ij}=\la A_i, B_j\ra \text{ where } A_1,..,A_n, B_1,..,B_m\in \psd^k,
%\ee
%for some $k \in \mathbb{N}$. The least $k$ for which  a PSD factorization exists is called the {\em PSD-rank} of $X$. 
%
%A couple of remarks. First, PSD factorizations generalize NMFs. Indeed,  nonnegative vectors  are in 1-1 correspondence with diagonal PSD matrices as follows:  $x\in \R^n_+ \mapsto {\rm diag}(x)$. In other words, a NMF factorization is a special case of a PSD factorization where all matrices $A_1,..,A_n, B_1,..,B_m$ are diagonal.  As a consequence, PSD factorizations always exists and furthermore, the PSD-rank is upper bounded by  the nonnegative rank. Calculating optimal PSD-factorizations
% is hard \cite{Shitov}. For more details see the survey \cite{PSDrank}.
%
%
%
%
%
%\subsection{Motivation I}Analogously  to the case of nonnegative rank, the PSD-rank of the slack matrix of a polytope expresses the smallest size of a semidefinite program that captures the polytope. Specifically:
%
%
%
%\begin{theorem}\cite{psdlifts} Consider a polytope 
%$$P=\{x: Ax\le b\}={\rm conv}(v_1,..,v_m).$$ Let $S_P$ be the  {\em slack matrix} of $P$, i.e., the matrix whose rows are indexed by the facets of $P$, its columns by its vertices,  and  $S_{ij}=b_i-\la A_{i\cdot},v_j\ra$.   Then, the PSD-rank of $S_P$ is equal to the smallest $k\in \mathbb{N}$ for which 
%$$P=\pi(\psd^k \cap \mathcal{L}),$$
%where  $\mathcal{L}$ is an affine subspace of the space of $k\times k$ symmetric matrices. 
%\end{theorem}
%
%Roughly speaking, this theorem shows  that the PSD-rank captures the ``expressive power  of semidefinite programming''.
%

%
%Let's focus in the following sub-problem:  Let $\mathbb{S}^{n}$ denote the vector space of $n \times n$ symmetric matrices.  Let $B \in \mathbb{S}^{n}$ be positive semidefinite.  Let $\mathcal{A} : \mathbb{S}^{n} \rightarrow \mathbb{R}^{d}$ be a linear map.  Suppose $\bx \in \mathbb{R}^{d}$ is a non-negative vector.  Our goal is to compute a positive definite matrix $\tilde{B}$ such that
%\begin{equation*}
%	\mathcal{A} (\tilde{B}) \approx \bx.
%\end{equation*}
%The matrix $B$ represents our current estimate while $\tilde{B}$ represents our next iterate.  We wish to develop a cheap procedure that allows us to obtain a better solution $\tilde{B}$ building off $B$.
\fi

==> manuscript PSD case: arxiv/sec_nmf.tex <==
\section{Applications of the MMU algorithm}\label{sec:applications}
\paragraph{Block-diagonal (BD) PSD factorizations.} If the  MMU algorithm is initialized with~BD  positive definite   matrices  with   {\em the same} block structure, the  BD structure is preserved at each update. %  Such factorizations are relevant for the study of hybrid classical-quantum correlation generation~protocols. 
Indeed, as $[\mathcal{A}^{\sfT} \mathcal{A}] (\bo)=\sum_{k=1}^m\tr( A_k\bo) A_k$ we see that $[\mathcal{A}^{\sfT} \mathcal{A}] (\bo)^{-1}$, and thus, $([\mathcal{A}^{\sfT} \mathcal{A}] (B_j))^{-1}\#(B_j)$ share the same block structure. Lastly, by definition of  the MMU algorithm~\eqref{updaterule}, $\bn$ is also  block-diagonal with the same structure. Thus, 
 if initialized with~BD-PSD matrices, the MMU algorithm  gives a method for computing a BD-PSD factorization.%, which are relevant for the study of hybrid classical-quantum correlation generation~protocols. 
%Thus, if  initialized witha BD  positive definite matrices,  the MMU algorithm   is the first method   for calculating block-diagonal PSD factorizations, which as described in the introduction,  are relevant for the study of hybrid classical-quantum correlation generation~protocols. 
%

\paragraph{Recovering  Lee-Seung's algorithm for NMF.} Diagonal matrices can be considered as  block-diagonal in a  trivial manner. Nevertheless, by the preceding discussion, if initialized with diagonal PSD matrices, the iterates of the MMU algorithm remain diagonal PSD throughout. In this special case, our MMU algorithm  
reduces to   Lee-Seung's~(LS) seminal Multiplicative Update algorithm  for   computing NMFs \cite{LS00}.  LS's algorithm is perhaps the most widely used  method for computing  NMFs    as it has succeeded to identify  meaningful features in  a diverse collection of real-life data sets and is extremely   simple  to implement. Specifically, LS's  updates are
\be\label{LSalg}
A\leftarrow  A \circ {XB^\top \over ABB^\top} \ \text{ and } \  B\leftarrow  B\circ {A^\top X\over A^\top A B},
\ee
where $X\circ Y, X/Y$ denote  the componentwise multiplication, division of two matrices respectively. Setting $A_i={\rm diag}(a_i)$ and $B_j={\rm diag}(b_j)$,  %$$W^{-1}={\rm diag}(b_j)^{-1}\#[\mathcal{A}^{\sfT} \mathcal{A}] ({\rm diag}(b_j))={\rm diag}(b_j)^{-{1\over 2}}\left(\sum_{i=1}^m \la a_i, b_j\ra {\rm diag}(a_i)\right)^{1\over 2},
%$$
%%$$[\mathcal{A}^{\sfT} \mathcal{A}] (\bo)=%\sum_{i=1}^m \tr({\rm diag}(a^{\new}_i){\rm diag}(\sbo)){\rm diag}(a^{\new}_i)=
%%\sum_{i=1}^m \la a_i^{\new}, \sbo\ra {\rm diag}(a^{\new}_i).
%%$$
%where we used the definition of the geometric mean  \eqref{GM} and the fact that $(AB)^{1\over2}=A^{1\over2 }B^{1\over 2}$ for positive commuting matrices. %we immediately get that 
%%$$Q=\bo^{-1/2}[\mathcal{A}^{\sfT} \mathcal{A}] (\bo)^{1\over 2}.$$
%Consequently, 
the MMU algorithm updates $B_j$ as
$$
B_j \leftarrow B_j\Big(\sum_{i=1}^m \la a_i, b_j\ra A_i\Big)^{-1}\Big(\sum_{i=1}^mX_{ij}A_i\Big),
%\bo[\mathcal{A}^{\sfT} \mathcal{A}] (\bo)^{-1}\mathcal{A}^\sfT(x)
$$
 which is also a diagonal PSD matrix. Setting $A^\sfT =\begin{pmatrix} a_1^\sfT & \ldots & a_m^\sfT \end{pmatrix}$ and $ B=\begin{pmatrix}b_1 & \ldots & b_n \end{pmatrix}$, we immediately recover  LS's  update rule~\eqref{LSalg}. 
%and furthemore 

%
%Letting  $\bn=[\sbn_1\ldots \sbn_n]$ it will be useful to equivalently express  the Lee-Seung updates with respect to the columns of $\bn$ (and similarly for $\an$), i.e.,  
%%$$\sbn_j(k)=\sbo_j(k) {\an^\sfT X_{:j} \over \an^\top \an\sbo_j }.$$
%\be\label{vdbdfg}
%\sbn_j(k)=\sbo_j(k) {\sum_{i=1}^m\san_i(k)X_{ij} \over \sum_{i=1}^m\san_i(k)\la \san_i,\sbo_j\ra}.
%\ee
% We now show that the Lee-Seung algorithm can be recovered as a special case of our framework for finding PSD factorizations, when restricted to diagonal PSD matrices. 
%For this, recall that an equivalent way of expressing the NMF  problem  is  to find   two families of nonnegative vectors $\{a_i\}\subseteq~\R^r_+$ and $\{b_j\}\subseteq  \R^r_+$  satisfying $
%X_{ij}= \la a_i,b_j\ra,$ for all $  i\in [m],\ j\in [n]$. Furthermore, note that nonnegative vectors can be isometrically mapped to PSD matrices by the diagonalization  operator $x\mapsto {\rm diag}(x)$. 
%Consequently, NMF corresponds to special case of the PSD factorization problem, when we restrict to PSD factors that are diagonal. It remains  to show that in this case, the iterates generated by our algorithm for PSD factorizations are also PSD diagonal, and in fact, they coincide with the iterates generated by the Lee-Seung algorithm. 
%

%
%Thus, we can try to find  an (approximate) NMF  by solving the nonconvex optimization problem 
%\be\label{cdsvds}
%\inf \left\{{1\over 2}\sum_{i,j}(X_{ij}-\la a_i,b_j\ra)^2: \ a_i, b_j\in \R_+^r  \right\}.
%\ee
%As in the PSD case, problem \eqref{cdsvds} can be  solved using  an alternate minimization approach, where we alternate between updating the $a_i$'s and $b_j$'s. Concretely, assuming the $a_i$'s have been updated to $a_1^{{\rm new}}, \ldots, a_m^{{\rm new}}$ and considered   fixed, the problem is separable with respect to each vector variable $b_j$ and thus, omitting indices for clarity of presentation, it suffices to solve the~problem:
%\be\label{vsvsdfv}
% \inf \left\{{1\over 2}\|x-\mathcal{A}(b)\|^2: \  b \in \R^r_+  \right\},
%\ee
%where 
%$\mathcal{A} : \R^{r} \rightarrow \mathbb{R}^{m}$ is the linear map 
%\begin{equation*}
%	\mathcal{A}(z) = \left(
%	\langle a_1^{{\rm new}},z \rangle, \ \ldots \ 
%	,\langle a_m^{{\rm new}},z \rangle
%	 \right). 
%\end{equation*}
%Note that \eqref{vsvsdfv} is a special case of the subproblem we encountered in the PSD case (recall  \eqref{main}),  the only difference being that the matrices $A_i$ are now diagonal PSD matrices. 


\paragraph{PSD factorizations for nonnegative tensors.}  Motivated by PSD factorizations of nonnegative matrices,  \cite{tensor} define  an $r$-dimensional  PSD factorization of a nonnegative tensor $T$ (with $n$ indices of dimension $d$) as a collection of PSD matrices $C^{(1)}_{i_1}, \ldots, C^{(n)}_{i_n} \in \psd^r $ for all $i_k\in [d]$  such that
  \be\label{tensor}
     T_{i_1, \ldots, i_n} = \sum_{i, j=1}^r C^{(1)}_{i_1}(i,j) \cdots C^{(n)}_{i_n}(i,j), \  \text{ for all } i_k \in [d].
     \ee%={\rm sum}(C_{x_1}\circ \ldots \circ C_{x_k}),
Equivalently, and more succinctly, we may write \eqref{tensor} as 
$$   T_{i_1\ldots i_n}={\rm sum}(C^{(1)}_{i_1}\circ \cdots \circ C^{(n)}_{i_n}),  \text{ for all }  i_k \in [d], $$ where $\circ $ denotes the Schur product of matrices and ${\rm sum}(X)=\sum_{ij}X_{ij}$. The motivation for studying tensor PSD factorizations  comes from the fact that they characterize   the quantum correlation complexity for generating multipartite classical distributions \cite{tensor}. 
  We now show how our MMU algorithm can be used as a primitive to calculate tensor  PSD factorizations.  
   For simplicity of presentation we restrict  to  $n=3$     and~consider
    \be\label{vsvs}
    \inf  \sum_{i_1, i_2, i_3}\left( T_{i_1 i_2i_3} -{\rm sum}(C^{(1)}_{i_1}\circ C^{(2)}_{i_2} \circ C^{(3)}_{i_3})\right)^2  \quad  \text{subject to} \quad  C^{(1)}_{i_1}, C^{(2)}_{i_2},  C^{(3)}_{i_3} \in \psd^r.
    \ee
   As in the case of PSD factorizations, to solve \eqref{vsvs} we employ a block coordinate descent approach. Specifically,  fixing all matrices $C^{(1)}_{i_1}, C^{(2)}_{i_2}$ the optimization problem \eqref{vsvs} is separable wrt each $C^{(3)}_{i_3}$ for all $i_3\in~[d].$ 
  Thus,   we need to solve the optimization problem
    \be\label{vsf}
    \arg \inf_C \sum_{i_1, i_2}\left(T_{i_1 i_2i_3} - \langle C^{(1)}_{i_1}\circ C^{(2)}_{i_2}, C\rangle\right)^2 \quad  \text{ subject to } \quad C\in \psd^r.
    \ee
Defining the  map  $\mca: \mathbb{S}^r \to \mathbb{R}^{d^2}$ where $  X\mapsto (\la X, C^{(1)}_{i_1}\circ C^{(2)}_{i_2}\ra)_{i_1,i_2} $, problem \eqref{vsf} is 
equivalent to
\be\label{csvsdv}
\arg \inf \|{\rm vec}(T_{::i_3})-\mca(C)\|^2_2 \quad \text{ subject to} \quad C\in \psd^r,
\ee
for all $i_3\in [d]$. Note that $\mca^\sfT: \mathbb{R}^{d^2} \to  \mathbb{S}^r $ where $   x=(x_{x_1x_2})\mapsto \sum_{i_1, i_2\in [d]}x_{i_1i_2}C^{(1)}_{i_1}\circ C^{(2)}_{i_2} $ is a PSD matrix, as the Schur product of PSD matrices is PSD. Thus,  Theorem \ref{LSstylethm} gives  an update rule that preserves PSDness and  for which the objective function \eqref{csvsdv}  is nonincreasing.% The analogous algorithm for computing NMF's of nonnegative tensors that use LS's as a primitive was given in~\cite{PTF}. 


==> manuscript PSD case: arxiv/sec_numexp.tex <==
\section{Numerical experiments}\label{sec:numerical}

\paragraph{Distance matrices.}  %Our first numerical experiment applies the MWU algorithm to compute  a PSD factorization of a distance matrix.  
Let $v \in \mathbb{R}^{n}$ be a vector and let $M$ be a $n\times n$ matrix whose entries are $M_{ij} = (v_i-v_j)^2$.  $M$ is known as a \emph{distance matrix} and a 2-dimensional PSD factorization is  $M_{ij} = \mathrm{tr}(A_i B_j)$, where
$A_i = \left(\begin{smallmatrix}1 \\ v_i \end{smallmatrix}\right) \left(\begin{smallmatrix} 1 \\ v_i \end{smallmatrix}\right)^\sfT $ and $ 
B_j = \left(\begin{smallmatrix} -v_j \\ 1 \end{smallmatrix}\right) \left(\begin{smallmatrix} -v_j \\ 1 \end{smallmatrix}\right)^\sfT. $
We generate a random  $v \in \mathbb{R}^{n}$ with $n=20$ where each entry is drawn from the standard normal distribution.  We apply our algorithm to compute a 2-dimensional  factorization whereby we perform $500$ iterations over $50$ random initializations.  For conditioning reasons, we perform a damped update whereby we add $\epsilon I$, $\epsilon = 10^-8$, to each matrix variable at every iterate.  We compute the normalized squared error loss of the factorization from the data matrix, and we plot the error over each iteration $\mathrm{Err} =  \sum_{i,j} (\mathrm{tr}( A_i B_j ) - M_{ij} )^2 /\sum_{i,j} M_{ij}^2$  in Figure \ref{fig:distancematrx_errors}.
%As we supplied the correct PSD-rank to our algorithm, the smallest possible error is equal to zero.  %We note that while the error approaches zero in some cases, the eventual error is typically quite far from zero in many others.  
Our experiments  suggest that, with sufficient random initializations, our algorithm finds a PSD factorization that is close to being exact. %but the number of random initializations required may be prohibitively high if the dimension of the problem ($n$ in this instance) is moderately high.

\begin{figure}[h!]
\centering
\includegraphics[width=0.4\textwidth]{images/DM_err}
\includegraphics[width=0.4\textwidth]{images/DM_logerr}
\caption{Performance of the MWU algorithm for computing a PSD factorization of a distance matrix.  Different curves correspond to different random initializations. }% The MMU  algorithm computes a factorization with error close to zero for some initializations, which is the analytical solution
 % The left graph shows the squared error loss and the right graph shows the same  curves on the log scale.}
\label{fig:distancematrx_errors}
\end{figure}



%[IF THE THEOREM IS TRUE, THEN WHY ISN'T THE RANK OF $M$ EQUALS TO 2?] Consider the $n\times n$ matrix  with entries given by $M_{ij}=(i-j)^2.$ As $M$ is the Schur product of $S_{i,j}=(i-j)$ which has rank 2, it follows that the psd-rank of $M$ is at most 2. Furthermore,  for $k\in \{1 ,2\}$ we have that $\rank(A)=k \Longleftrightarrow  \psdrank(A)=k$ \cite{psdrank}. As the rank of $M$ is 3 as can be seen from the factorization $M_{ij}= (i^2, -2i, 1)^\sfT (1, j, j^2)$ for all $i,j\in [n]$.it follows that the psd-rank of $M$ is 2.  

\paragraph{CBCL Face Image Dataset.}  In our second  experiment we apply  the MMU  method to compute a PSD factorization  of face image data from the CBCL Face Database \cite{CBCL}. 
The objective of this experiment is to explain how computing a PSD factorization can be viewed as a representation learning algorithm that generalizes NMF.  %Our numerical experiment expands upon a similar experiment on the same dataset but using NMF \cite{LS99}. 
 The CBCL dataset comprises $2429$ images of faces, each of size $19 \times 19$ pixels,  linearly scaled so that the pixel intensity has mean $0.5$ and standard deviation $0.25$, with values  subsequently clipped at $[0,1]$.  The resulting data matrix has size $361 \times 2429$.   Our experiments were conducted in Python on an Intel 7-th Gen i7 processor at 2.8GHz.

 
Recall that    an $r$-dimensional PSD factorization   of $X$ given by   $\{A_i\}, \{B_j\}$ 
 gives rise   to a representation  
$X_{:j}=\sum_i\lambda_i\cala(u_iu_i^\sfT)$, where  $B_j=\sum_{i=1}^r\lambda_iu_iu_i^\sfT$ is the  spectral decomposition  
of~$B_j$ and $\cala: \mathbb{S}^r \to \R^m$ is the   linear mapping satisfying $Z\mapsto (\tr(A_1Z), \ldots, \tr(A_mZ)).$
In all figures in this section, given a specific image $X_{:j}$ in the CBCL dataset, we illustrate the images corresponding to the building  blocks identified by the MMU algorithm, namely $\cala(u_iu_i^\sfT)$ for all eigenvectors of $B_j$.
 

%Concretely, suppose we compute a NMF of the data matrix $X \approx AB^{T}$.  The factor $A$ can be interpreted as a basic collection of face images in that every face in the dataset is well approximated as $AB_{i:}^T$ (for some $i$).  In particular, the face is approximated as a \emph{non-negative} linear combination of the columns of $A$ whose weights are given by the vector $B_{i:}$. 
 As our baseline, we compute a 27-dimensional  NMF of the CBCL data matrix  over $500$ iterations. In Figure \ref{fig:1x1_full} below 
 % The factor $A$ has $27$ columns, 
 we illustrate  the decomposition of one of  images from  the dataset  into these $27$ constituents. 
 
\begin{figure}[h]
\centering
\includegraphics[width=1\textwidth]{images/1x1_full}
\caption{Image decomposition into  building blocks learned from 27-dimensional NMF.}
\label{fig:1x1_full}
\end{figure} 
Next, we calculate a 7-dimensional PSD factorization of the CBCL data matrix over 500 iterations and 
illustrate the decomposition of the same image in the new basis in Figure \ref{fig:PSD_full}. 
  %the analogous decomposition of a face image using a PSD factorization of size $7\times 7$ over $500$ iterations. 
   We compute a factorization of size $7$ to match the number of degrees of freedom in Figure \ref{fig:1x1_full}.
%Suppose we compute a PSD factorization of the data matrix $X \approx \mathcal{A} \mathcal{B}^{T}$ instead.  Then every face image is of the form $\mathcal{A}(\mathcal{B}_{i:})$, where $\mathcal{B}_{i:}$ is a PSD matrix rather than a non-negative vector.  Compute the spectral decomposition so that $\mathcal{B}_{i:} = \sum \sigma_k u_k u_k^{\sfT}$.  Then $\mathcal{A}(\mathcal{B}_{i:}) = \sum \sigma_k \mathcal{A}(u_k u_k^{\sfT}) $.  Notice that $\sigma_k \geq 0$, and hence if we view the elements of the form $\mathcal{A}(E)$ where $E$ is a unit-norm rank one matrix as basic building blocks, then the approximation $\mathcal{A}(\mathcal{B}_{i:})$ is also a non-negative linear sum of such constituents.
We note that the constituents learned from the PSD factorization  are less interpretable than those learned using~NMF -- here, we use the word `interpretable' in a loose sense to mean that some factors learned from NMF are easily interpreted to describe local facial features such as the eyes or the nose whereas the constituents learned from PSD are of a global nature. Nevertheless, we note that this  phenomenon that has been  been also observed for NMF applied to  datasets beyond  CBCL \cite{nonatomicNMF}. 
\begin{figure}[h]
\centering
\includegraphics[width=1\textwidth]{images/PSD_full}
\caption{Image decomposition  into  building blocks learned from 7-dimensional PSD factorization.}
\label{fig:PSD_full}
\end{figure}

%
%
%are less interpretable than those learned using NMF -- here, we use the word `interpretable' in a loose sense to mean that some factors learned from NMF are easily interpreted to describe local facial features such as the eyes or the nose whereas the constituents learned from PSD Nevertheless, 
%
%
%One explanation is that the decomposition of a matrix into rank-one components is \emph{not} unique.%\footnote{The \emph{spectral} decomposition is unique only if we impose the addition constraint that the rank-one components are \emph{orthogonal}.} 

 %Building on the ideas described in Section [REF], we can instead learn 
 Lastly, we use the MMU algorithm to %learn a PSD factorization with block-diagonal structure. 
 %blending  the interpretability from NMF with the ability to express infinitely many basis elements via PSD factorizations. 
 %As an illustration, we 
 compute a block-diagonal PSD factorization with  $9$ blocks, each  of size $2$, over $500$ iterations (the number of degrees of freedom is comparable), which we illustrate the decomposition in Figure \ref{fig:2x2_full}.  In this instance, the constituents contain more localized~features.  
 
 \begin{figure}[h]
\centering
\includegraphics[width=1\textwidth]{images/2x2_full}
\caption{Image decomposition  into  building blocks learned using  $2\times 2$-block PSD factorization.}
\label{fig:2x2_full}
\end{figure}
 
 
 An advantage of learning a continuum of basic building blocks is that one can express certain geometries in the data that is otherwise not possible using a finite number of building blocks -- as an illustration of this intuition, in Figure \ref{fig:2x2_atoms}, we show a continuum of atoms corresponding to a single $2\times 2$ block, which  capture a continuum between the nose and the nostrils.


 %Despite this success, there also exist data sets for which NMF does not give an intuitive decom- position into parts that would correspond to our idea of the ‘building blocks’ of the data. 


%In fact, computing a PSD factorization of the face data matrix may be interpreted as computing an \emph{infinite} collection of basic building blocks for describing faces.  To simplify our explanation, we first describe the analog using NMF.  Specifically, in NMF, we approximate the data matrix as $AB^{T}$, where $A$ and $B$ are non-negative factors.  Then the columns of $A$ are basic building blocks for describing faces, and every face in the dataset is well approximated as the non-negative linear sum of these building blocks -- Figure \ref{fig:face_NMFfactorization} illustrates this example.  In PSD factorization, each face is non-negative linear sum of building blocks of the form $\mathcal{A}(E)$ where $E = \bu \bu^{\sfT}$ is a unit-norm rank-one positive semidefinite matrix -- we illustrate this in Figure \ref{fig:face_PSDfactorization}.  The elements $\mathcal{A}(E)$ is the analog of a column of $A$ in NMF.  To see this, note that a column of $A$ in NMF can be viewed as $A \boldsymbol{e}_j$, where $\boldsymbol{e}_j$ is a standard basis vector, and that the analog in PSD factorization is to replace $\boldsymbol{e}_j$ with a unit-norm rank one PSD matrix.

% The images of the form $\mathcal{A}(E)$ where $E = \bu \bu^{\sfT}$ is a unit-norm rank-one positive semidefinite matrix can be viewed as a learned collection of basic atoms to build a face image.  Subsequently, every face image $\bx_j$ is a \emph{non-negative linear sum} of these atoms.  While NMF seeks a \emph{finite} collection of basic elements, constrained to take non-negative values, from which every data can be expressed as non-negative sums, PSD factorization seeks an \emph{infinite} collection of such basic elements as there are infinitely many rank-one matrices.

%In Figure \ref{fig:face_factorization}, we show a subset of basic elements of the form $\mathcal{A}(E)$, where $E$ are randomly chosen unit-norm rank-one matrices of the form $E = \bu \bu^{\sfT}$, with $\bu$ drawn from the uniform measure over the set of vectors with norm equals to one.  

%\begin{figure}
%\centering
%\includegraphics[width=0.40\textwidth]{images/faces_sample}
%\hspace{10mm}
%\includegraphics[width=0.40\textwidth]{images/faces_array}
%\label{fig:face_factorization}
%\caption{Computing a PSD factorization of a Face Image Dataset.  The left sub-figure shows samples from the dataset and the right sub-figure shows the basic elements learned computing a PSD factorization -- these are linear images of learned LHS factor applied to rank-one matrices.}
%\end{figure}







\begin{figure}[h!]
\centering
\includegraphics[width=1\textwidth]{images/2x2_atoms}
\caption{Visualization of continuum of  building blocks learned using $2\times 2$-block PSD factorization.}
\label{fig:2x2_atoms}
\end{figure}

\paragraph{Acknowledgments.}  YS gratefully acknowledges Ministry of Education (Singapore) Academic Research Fund (Tier 1) R-146-000-329-133.  AV gratefully acknowledges Ministry of Education (Singapore) Start-Up Research Grant SRG ESD 2020 154 and NRF2019-NRF-ANR095 ALIAS grant. 

%\medskip 


%\paragraph{Correlation polytope:} 
%  The correlation polytope is given by ${\rm conv}(bb^\sfT: b\in \{0,1\})$. For any $a\in \{0,1\}^n$,   a valid inequality for the correlation polytope is given by: 
%$$ \la 2{\rm diag}(a)-aa^\sfT,x\ra\le 1.$$
% Indeed,    substituting  $x=bb^\sfT$  we get that $$(a^Tb-1)^2\ge 0, $$ where we use that $b\in \{0,1\}^n$ and thus $b_i^2=b_i$.
%We consider the  slack matrix $S$ corresponding to these valid inequalities; its rows and columns are  indexed by $a,b\in \{0,1\}^n$ and has  entries:
%$$S_{a,b}=(a^\sfT b-1)^2=\la \begin{pmatrix} 1&  -a \end{pmatrix} \begin{pmatrix} 1&  -a \end{pmatrix} ^\sfT,  \begin{pmatrix} 1&  b \end{pmatrix}  \begin{pmatrix} 1&  b\end{pmatrix} ^\sfT \ra, $$
%Consequently, the psd-rank of $S$ is at most $n+1$ (and the psd factors have rank 1). 
%

%Here we discuss two algorithms for NMF based on iterative updates ofWand H. Because these algorithms are easy to implement and their convergence properties are guaranteed, we have found them very useful in practical applications. Other algorithms may possibly be more efficient in overall computation time, but are more difficult to implement and may not generalize to different cost functions.





%This update rule seems to work well in numerical experiments.  

%In the first case, consider a synthetic example.  The matrix $X = \mathcal{A}\mathcal{B}^{\sfT}$ is a non-negative matrix with some low-rank PSD factorization.  The algorithm is initialized with some random linear maps, and the graph plots the error $\| \mathcal{A}_{t}\mathcal{B}_{t}^{\sfT} - X \| $.  

%\begin{figure}[h]
%	\centering
	%\includegraphics[width=0.50\textwidth]{psd_errors.png}
%	\label{fig:graph1}
%	\caption{Norm errors.  The red curve marks the errors using the proposed method.  The other curves are previous attempts.}
%\end{figure}

%Here's a different example where $X$ is just a generic matrix with positive entries, and so the global solution is greater than zero.

%\begin{figure}[h]
%	\centering
	%\includegraphics[width=0.50\textwidth]{psd_generic.png}
%	\label{fig:graph1}
%	\caption{Norm errors.  The red curve marks the errors using the proposed method.  The other curves are previous attempts.  Red curve beats the other methods (marginally), which is a good sign.}
%\end{figure}



==> sec_checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage

\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerNo{}  
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}  %Our work is foundational and it informs the development for other machine learning frameworks such as neural networks (and especially CNNs).  We have decided to not include a discussion on potential societal impacts because (i) the discussion will be highly speculative, which distracts from the important purpose such discussions serve, and (ii) future downstream applications that build on our framework is the most reasonable 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}  The proof of Theorem \ref{LSstylethm} is in the main body.  It relies on Lemma \ref{thm:domination_general}, which is stated and proved in the Appendix.  The proof of Theorem \ref{fixedpointsthm} is found in the Appendix.
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}  The essential instructions are provided in the numerical experimental section.  The code will be uploaded to an online repository at a later date. 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}  An important feature of the MMU (our) algorithm we propose is that it does \emph{not} require a tuning parameter.  In the numerical experiment on the CBCL Face dataset, the choice of parameters were such that the number of degrees of freedom in all three methods are similary (either 27 or 28).
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}  The PSD factorization task is non-convex so the performance of any algorithm is dependent on initialization.  We describe the error bars (indirectly) in our plot in Figure \ref{fig:distancematrx_errors}.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}  The experiments were conducted on a laptop, and we briefly state the specifications in the mainbody.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} We used the CBCL Face Dataset \cite{CBCL}.
  \item Did you mention the license of the assets?
    \answerNo{}  We do not mention the license because it appears to be customized.  Nevertheless the license permits use of the dataset for academic research, and can be found on the cited URL.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}



==> sec_existing.tex <==
\section{Prior works on computing PSD factorizations}
All 
existing algorithms for computing PSD factorizations  employ the alternating minimization approach described in the previous section, where we fix one set of variables and minimize over the other, and essentially boil  down into finding algorithms for  the convex problem \eqref{main}.

% In the following, we discuss prior works for minimizing \eqref{bigboss} by focusing on the following sub-problem:
%\be\label{small}
%\inf \Big\{\|x-\mathcal{A}(B)\|^2: \  B \in \psd^r  \Big\}.
%\ee

\paragraph{Projected Gradient Method (PGM).}  The first approach for computing PSD factorizations  is based on  applying PGM to \eqref{main}, alternating  between a gradient step to minimize the objective and  a projection step onto the set of PSD matrices \cite{VGG18}.  The latter projection step uses the following useful fact: Given the spectral decomposition $C=U{\rm diag}(\lam_i)U^\sfT$ of a matrix $C\in \bbS^n$, the projection onto the PSD cone is $U{\rm diag}(\max(0,\lam_i))U^\sfT$ \cite{hig}.  The vanilla PGM has slow convergence rate, so the authors in \cite{VGG18} also propose an accelerated variant that incorporates a momentum term.

\paragraph{Coordinate Descent.}  The authors in \cite{VGG18} also propose a different algorithm combining the ideas of coordinate descent and  a change of variables that allows them to also control  the rank of the PSD factors, which  was popularized by  the seminal work of Burer and Monteiro for solving rank-constrained SDPs \cite{BM}. 
%explicitly expressing each factor in its PSD factorization to enforce the PSD constraint. 
  Concretely, the authors use the  parameterization  $A_i=a_ia_i^\sfT$, and $B_j=b_jb_j^\sfT$, where $a_i\in \R^{r\times r_{A_i}}$, and $b_j\in \R^{r\times r_{B_j}}$ for some fixed $r_{A_i}, r_{B_j}\in \mathbb{N}$, and optimize using a coordinate descent scheme over  the entries of the matrices $a_i$ and $b_j$.
  %  This approach is frequently associated  with  the seminal work of Burer and Monteiro for solving rank-constrained SDPs \cite{BM}, and has the advantage that the matrices $A_i$ and $B_j$ may be rank deficient. %The BM approach relies on the observation that  an  $n$-by-$n$ psd matrix $X$ with rank $r$ can be written as $X=\sum_{i=1}^rx_ix_i^\sfT=XXT$ for some real vectors $x_1,\ldots, x_r\in \R^{n\times 1}$. 
%Specifically, fixing (in some ad-hoc manner) the ranks $r_{A_i}$ and $r_{B_j}$ for each $A_i$ and $B_j$ respectively, it follows that there exists matrices $a_i\in \R^{r\times r_{A_i}}$ and  $b_j\in \R^{r\times r_{B_j}}$ such that  $A_i=a_ia_i^\sfT$ and $B_j=b_j{b_j}^\sfT$.  
Thus,  problem \eqref{main}~becomes: 
\be\label{BM}
 \underset{b}{ \inf} ~~ \| x - \mathcal{A} (bb^\sfT) \|_2^2 \quad \mathrm{s.t.} \quad  b\in \R^{r\times r_B},
 \ee
which is a quartic polynomial in the entries of $b$.  Thus, its gradient is a cubic polynomial, 
%as the following problem over the $a_i$'s and $b_j$'s:
%\be\label{factorformulation}
%{\inf} \Big\{ \sum_{i,j}(X_{ij}-a_i^\sfT b_j)^2: \ a_i\in \R^{r\times r_{A_i}},  b_j\in \R^{r\times r_{B_j}}\Big\}.
%\ee 
%The algorithm proceeds by fixing one set of variables -- say the $a_i$'s -- while updating the other set -- say the $b_j$'s.  The resulting problem entails the minimization of a degree four polynomial over $\R_+$, 
and its roots can be found  using  Cardano's method (and careful book-keeping). %an explicit formula for  the roots of a cubic polynomial (as Cardano's method).
 
% We conclude with a note on the convergence properties of the coordinate descent method: Every limit point of the sequence of iterates generated by the CD method is a stationary  point if the minimum in each CD subproblem is uniquely attained (assuming a convex objective function and convex constraint sets) \cite{Ber}.  Nevertheless, note that these assumptions are not necessarily satisfied in this case.   Lastly, we note that  an additional desirable  feature of the factor-based formulation~(\eqref{factorformulation}) is that   it allows to explicitly  control the rank  of the PSD factors, i.e., the $r_j$'s. 


\paragraph{Connections to Affine Rank Minimization and Phase Retrieval.}  A different set of algorithms developed in \cite{LF20, LF20b, LLTF20} is based on the connections between computing PSD factorizations with the affine rank minimization (ARM) and the phase retrieval (PR) in signal procesing.  
First, recall that the PSD-ARM problem focuses on  recovering a low-rank matrix from affine measurements:
$$
 \min_B ~~ \rank(B) \quad \text{s.t.} \quad   \ \cala(B)=x, \ B\in \psd^r.
$$
Here, $\cala$ is a known linear map representing measurements while $x$ is known vector of observations. Due to the non-convexity of the rank function, a useful heuristic initially popularized in the control community  is to replace the rank by  the trace function, e.g., see \cite{MP} and \cite{fazel}, in which case the resulting problem is an instance of an SDP.  A different  heuristic for   PSD-ARM is to find a PSD matrix of rank at most $k$ that  minimizes the squared loss function, i.e., \be\label{cdsfvsdfv}
 \inf~~ \|x-\cala(B)\|_2^2 \quad \text{s.t.} \quad  B\in \psd^r, \ \rank(B)\le k,
\ee
where alternatively, the rank constraint can be enforced  by parametrizing the PSD matrix variable $B\in \psd^r$ as $B=bb^\sfT$ with $b\in \R^{r\times k}$. 
The point of departure for the works  \cite{LF20, LLTF20, LF20b} is that problem~\eqref{cdsfvsdfv}  corresponds exactly to  the sub-problem \eqref{main} encountered in any alternate minimization strategy for computing  PSD factorizations,   albeit with an additional  rank constraint. In view of this, any  algorithm  from the signal processing literature developed for ARM can be applied to \eqref{main}.


%can be optimized using existing methods in the literature that were developed for phase retrieval and ARM.

The main algorithms considered in \cite{LF20, LF20b, LLTF20}  are Singular Value Projection (SVP)  \cite{SVP},   Procrustes Flow \cite{procrsustes}, and variants thereof.
%which  involves an initialization phase   based on SVP  followed by a  second phase which  essentially performs gradient descent with a meticulously  chosen step size. 
In terms of convergence guarantees,  for affine maps $\mathcal{A}$  obeying the  Restricted Isometry Property \cite{RIP}, both algorithms converge to an optimal solution. Nevertheless, it is unclear whether these guarantees carry over when applied to the PSD factorization problem. 

%The link to the phase retrieval problem becomes apparent when   we restrict to   PSD factorizations with rank-1 factors,  i.e., $A_i=a_ia_i^\sfT$ and $B_j=b_jb_j^\sfT$, for some $r$-dimensional vectors $a_i, b_j$. In this setting, a PSD factorization of the data matrix $X$ can be interpreted as:
%$$X_{ij}\approx \mathrm{tr}( A_i B_j )=|\la a_i,b_j\ra|^2.$$
%Assuming as usual that  the $a_i$'s are fixed,   this is just the problem  of recovering a signal (the $j$-th column of $X$)  from phaseless
%measurements  given by the sensing vectors $a_1, \ldots, a_m$. 



%Lastly, note   that \eqref{small} is an instance of a convex quadratic semidefinite program, i.e., an optimization problem of the form:
%$$
%\min \{{1\over 2} \la X, \mathcal{Q}(X)\ra+\la C,X\ra:\ \mathcal{L}(X)=b, X\succeq 0 \},$$
%where $\mathcal{Q}: \mcs^n\to \mcs^n$  is a self-adjoint positive semidefinite linear operator on  (i.e., $\la X, \mathcal{Q}(X)\ra\ge~0, \forall X\in \mathcal{S}^n$), $b$ is a vector in $\R^m$ and $\mathcal{L}$ a linear mapping from $\mcs^n\to \R^m$. Indeed, in this case we have that $\mathcal{Q}=\cala\cala^\sfT$ which is psd as 
%$\la X, \mathcal{Q}(X)\ra=\|\cala(X)\|_F^2\ge0$.
%


